FirmwareDroid: Security Analysis of the Android Firmware EcoSystem

The Android Open Source Project (AOSP) is probably the most used and customized operating system for smartphones and IoT devices worldwide. Its market share and high adaptability makes Android an interesting operating system for many developers. Nowadays, we use Android firmware in smartphones, TVs, smartwatches, cars, and other devices by various vendors and manufacturers. The sheer amount of customized Android firmware and devices makes it hard for security analysts to detect potentially harmful applications. Another fact is that many vendors include apps from 3rd party developers. Such bloatware usually has more privileges than standard apps and cannot be removed by the user without rooting the device. In recent years several cases were reported where 3rd party developers could include malicious apps into the Android built chain. Media reports claim that pre-installed malware like Chamois and Triade we able to infect several million devices. Such cases demonstrate the need for better strategies for analyzing Android firmware. In our study, we analyze the Android firmware eco-system in various ways. We collected a dataset with several thousand Android firmware archives and show that several terabytes of firmware data are waiting on the web to be analyzed. We develop a web service called FirmwareDroid for analyzing Android firmware archives and pre-installed apps and create a dataset of firmware samples. Focusing on Android apps, we automated the process of extracting and scanning pre-installed apps with state of the art open-source tools. We demonstrate on real data that pre-installed apps are, in fact, a a threat to Android's users, and we can detect several hundred malware samples using scanners like VirusTotal, AndroGuard, and APKiD. With state of the art tools, we could scan more than 900000 apps during our research and give unique insights into Android custom ROMs.

==> assets/Tables/Androwarn_App_list_privacy <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"DisplayName","cspan":1,"rspan":1,"markup":[2,11]},{"value":"Filename","cspan":1,"rspan":1,"markup":[3,8]},{"value":"Packagename","cspan":1,"rspan":1,"markup":[2,11]},{"value":"MD5*","cspan":1,"rspan":1,"markup":[3,4]}],[{"value":"This application records audio from the 'MIC' source","cspan":4,"rspan":1,"markup":[2,52]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]}],[{"value":"My Verizon Services","cspan":1,"rspan":1,"markup":[3,19]},{"value":"MyVerizonServices.apk","cspan":1,"rspan":1,"markup":[3,21]},{"value":"com.verizon.mips.services","cspan":1,"rspan":1,"markup":[3,25]},{"value":"59049cf207598f10c9d9551b99fca31b","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"System UI","cspan":1,"rspan":1,"markup":[3,9]},{"value":"SystemUIGoogle.apk","cspan":1,"rspan":1,"markup":[3,18]},{"value":"com.android.systemui","cspan":1,"rspan":1,"markup":[3,20]},{"value":"c3738c06a61bfecb913393d671fde4a8","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Google Fi","cspan":1,"rspan":1,"markup":[3,9]},{"value":"Tycho.apk","cspan":1,"rspan":1,"markup":[3,9]},{"value":"com.google.android.apps.tycho","cspan":1,"rspan":1,"markup":[3,29]},{"value":"cdbbf2b11dbaeb15bb57374883b2c89f","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Phone","cspan":1,"rspan":1,"markup":[3,5]},{"value":"GoogleDialer.apk","cspan":1,"rspan":1,"markup":[3,16]},{"value":"com.google.android.dialer","cspan":1,"rspan":1,"markup":[3,25]},{"value":"9b89e9b64affdb0b0f3b8f23e100960d","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"This application reads the current location of the device","cspan":4,"rspan":1,"markup":[2,57]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]}],[{"value":"LTE Broadcast Manager","cspan":1,"rspan":1,"markup":[3,21]},{"value":"QAS_DVC_MSP.apk","cspan":1,"rspan":1,"markup":[3,15]},{"value":"com.qti.ltebc","cspan":1,"rspan":1,"markup":[3,13]},{"value":"9d2ed99d1d8c158a4dde4f9412c5d29c","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Carrier Services","cspan":1,"rspan":1,"markup":[3,16]},{"value":"CarrierServices.apk","cspan":1,"rspan":1,"markup":[3,19]},{"value":"com.google.android.ims","cspan":1,"rspan":1,"markup":[3,22]},{"value":"48e96d56bb2bf5d4838f01430a4c137e","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"My Verizon Services","cspan":1,"rspan":1,"markup":[3,19]},{"value":"MyVerizonServices.apk","cspan":1,"rspan":1,"markup":[3,21]},{"value":"com.verizon.mips.services","cspan":1,"rspan":1,"markup":[3,25]},{"value":"59049cf207598f10c9d9551b99fca31b","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Hidden Menu","cspan":1,"rspan":1,"markup":[3,11]},{"value":"SprintHM.apk","cspan":1,"rspan":1,"markup":[3,12]},{"value":"com.google.android.hiddenmenu","cspan":1,"rspan":1,"markup":[3,29]},{"value":"3bb40d71113c1285d2fcea186d6ca02a","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Google Play services","cspan":1,"rspan":1,"markup":[0,20]},{"value":"PrebuiltGmsCoreQt.apk","cspan":1,"rspan":1,"markup":[3,21]},{"value":"com.google.android.gms","cspan":1,"rspan":1,"markup":[3,22]},{"value":"326f6514b2559a7d19c9971a2da70a1b","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Google App","cspan":1,"rspan":1,"markup":[3,10]},{"value":"Velvet.apk","cspan":1,"rspan":1,"markup":[3,10]},{"value":"com.google.android.googlequicksearchbox","cspan":1,"rspan":1,"markup":[3,39]},{"value":"eb7566588d9cafac77e25cf9596a596e","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Settings","cspan":1,"rspan":1,"markup":[3,8]},{"value":"SettingsGoogle.apk","cspan":1,"rspan":1,"markup":[3,18]},{"value":"com.android.settings","cspan":1,"rspan":1,"markup":[3,20]},{"value":"90ebbff4001869a01235271b3b2e4c66","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Messenger","cspan":1,"rspan":1,"markup":[3,9]},{"value":"PrebuiltBugle.apk","cspan":1,"rspan":1,"markup":[3,17]},{"value":"com.google.android.apps.messaging","cspan":1,"rspan":1,"markup":[3,33]},{"value":"0acf2716400585bf13af03ce83949101","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"VZW_Multicast_MW","cspan":1,"rspan":1,"markup":[3,16]},{"value":"QAS_DVC_MSP_VZW.apk","cspan":1,"rspan":1,"markup":[3,19]},{"value":"com.qualcomm.ltebc_vzw","cspan":1,"rspan":1,"markup":[3,22]},{"value":"3756ba0b3f73cdfdc4b16070a19717a8","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"This application reads location information from all available providers (WiFi, GPS etc\\_)","cspan":4,"rspan":1,"markup":[2,90]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]}],[{"value":"Google Play services","cspan":1,"rspan":1,"markup":[3,20]},{"value":"PrebuiltGmsCoreQt.apk","cspan":1,"rspan":1,"markup":[3,21]},{"value":"com.google.android.gms","cspan":1,"rspan":1,"markup":[3,22]},{"value":"326f6514b2559a7d19c9971a2da70a1b","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Google","cspan":1,"rspan":1,"markup":[3,6]},{"value":"Velvet.apk","cspan":1,"rspan":1,"markup":[3,10]},{"value":"com.google.android.googlequicksearchbox","cspan":1,"rspan":1,"markup":[4,39]},{"value":"b9d8009cf051f96a91874b8c820a7106","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Chrome","cspan":1,"rspan":1,"markup":[3,6]},{"value":"Chrome.apk","cspan":1,"rspan":1,"markup":[3,10]},{"value":"com.android.chrome","cspan":1,"rspan":1,"markup":[3,18]},{"value":"508e65b15292c34f79680c896855f29a","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Maps","cspan":1,"rspan":1,"markup":[0,4]},{"value":"Maps.apk","cspan":1,"rspan":1,"markup":[3,8]},{"value":"com.google.android.apps.maps","cspan":1,"rspan":1,"markup":[3,28]},{"value":"15989c0bd5bc7593c984f38e51b25e41","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Android System WebView","cspan":1,"rspan":1,"markup":[0,22]},{"value":"WebViewGoogle.apk","cspan":1,"rspan":1,"markup":[3,17]},{"value":"com.google.android.webview","cspan":1,"rspan":1,"markup":[3,26]},{"value":"87923767a9e46b895413759dd29bf43f","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"This application captures video from the 'CAMERA' source","cspan":4,"rspan":1,"markup":[2,56]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]}],[{"value":"Google Play services","cspan":1,"rspan":1,"markup":[3,20]},{"value":"PrebuiltGmsCoreQt.apk","cspan":1,"rspan":1,"markup":[3,21]},{"value":"com.google.android.gms","cspan":1,"rspan":1,"markup":[3,22]},{"value":"326f6514b2559a7d19c9971a2da70a1b","cspan":1,"rspan":1,"markup":[3,32]}],[{"value":"Photos","cspan":1,"rspan":1,"markup":[3,6]},{"value":"Photos.apk","cspan":1,"rspan":1,"markup":[3,10]},{"value":"com.google.android.apps.photos","cspan":1,"rspan":1,"markup":[3,30]},{"value":"ec3b52291d88fd0489e600ceda14ecf5","cspan":1,"rspan":1,"markup":[3,32]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},null,{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontWeight":"400","fontStyle":"normal","textDecoration":"","color":"","backgroundColor":""}}]},"options":{"table_caption":"Androwarn categories grouped by unique apps. *Note: Only one MD5 hash shown to save space. ","table_label":"tab:Androwarn_AppsGrouped"}}

==> assets/Tables/Androwarn_NativeShort <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Androwarn message","cspan":1,"rspan":1,"markup":[1,17]},{"value":"App count","cspan":1,"rspan":1,"markup":[1,9]}],[{"value":"This application loads a native library","cspan":1,"rspan":1,"markup":[1,39]},{"value":"530","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"This application loads a native library: \n'Lcom/qualcomm/ltebc/LTEBCFactory;->getInstance()Lcom/qualcomm/ltebc/LTEBCFactory;'","cspan":1,"rspan":1,"markup":[1,125]},{"value":"106","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"This application loads a native library: 'imscamera.jni'","cspan":1,"rspan":1,"markup":[1,56]},{"value":"92","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application loads a native library: 'imsmedia.jni'","cspan":1,"rspan":1,"markup":[1,55]},{"value":"92","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application loads a native library: 'printspooler.jni'","cspan":1,"rspan":1,"markup":[1,59]},{"value":"136","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"This application loads a native library: \n'Ljava/lang/String;->valueOf(Ljava/lang/Object;)Ljava/lang/String;'","cspan":1,"rspan":1,"markup":[1,109]},{"value":"170","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"This application loads a native library: 'tensorflowlite.jni'","cspan":1,"rspan":1,"markup":[0,61]},{"value":"68","cspan":1,"rspan":1,"markup":[3,2]}],[{"value":"This application loads a native library: 'curve25519'","cspan":1,"rspan":1,"markup":[1,53]},{"value":"68","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application loads a native library: 'flash'","cspan":1,"rspan":1,"markup":[1,48]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application loads a native library: \n'Ljava/lang/System;->loadLibrary(Ljava/lang/String;)V'","cspan":1,"rspan":1,"markup":[1,96]},{"value":"28","cspan":1,"rspan":1,"markup":[1,2]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},null,{"style":{"fontWeight":"400","fontStyle":"normal","textDecoration":"","color":"","backgroundColor":""}}]},"options":{"table_caption":"Androwarn examples of native library detection on Android10 firmware.","table_label":"tab:AndrowarnNativeDetectionExamples"}}

==> assets/Tables/Androwarn_UNIX <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Androwarn message","cspan":1,"rspan":1,"markup":[1,17]},{"value":"App count","cspan":1,"rspan":1,"markup":[1,9]}],[{"value":"This application executes a UNIX command containing this argument:\n'Ljava/util/Arrays;->toString([Ljava/lang/Object;)Ljava/lang/String;'","cspan":1,"rspan":1,"markup":[1,136]},{"value":"136","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"This application executes a UNIX command containing this argument: \n'Ljava/lang/String;->valueOf(Ljava/lang/Object;)Ljava/lang/String;'","cspan":1,"rspan":1,"markup":[1,135]},{"value":"102","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"This application executes a UNIX command containing this argument: 'ipconfig /all'","cspan":1,"rspan":1,"markup":[0,82]},{"value":"102","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"This application executes a UNIX command","cspan":1,"rspan":1,"markup":[0,40]},{"value":"204","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"This application executes a UNIX command containing this argument: 'cat /proc/meminfo'","cspan":1,"rspan":1,"markup":[1,86]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: 'su -c ls'","cspan":1,"rspan":1,"markup":[0,77]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: 'top -n 1 -d 5'","cspan":1,"rspan":1,"markup":[0,82]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: '/system/bin/sync'","cspan":1,"rspan":1,"markup":[0,85]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: '2'","cspan":1,"rspan":1,"markup":[1,70]},{"value":"114","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"This application executes a UNIX command containing this argument: \n'Ljava/io/File;->getAbsolutePath()Ljava/lang/String;'","cspan":1,"rspan":1,"markup":[1,121]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: '1'","cspan":1,"rspan":1,"markup":[1,70]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: 'logcat -d'","cspan":1,"rspan":1,"markup":[1,78]},{"value":"68","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: 'logcat -t %d 9'","cspan":1,"rspan":1,"markup":[1,83]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: ' /system/bin/sh -c read  '","cspan":1,"rspan":1,"markup":[1,94]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: 'ping -c 1 -w 100 www_google_com'","cspan":1,"rspan":1,"markup":[1,100]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: 'ping -c 1 www_google_com'","cspan":1,"rspan":1,"markup":[1,93]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: 'ping6 -c 1 www_google_com'","cspan":1,"rspan":1,"markup":[0,94]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: '/system/bin/getprop fakeTimestamp'","cspan":1,"rspan":1,"markup":[1,102]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: '0'","cspan":1,"rspan":1,"markup":[1,70]},{"value":"80","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: \n'Ljava/lang/StringBuffer;->toString()Ljava/lang/String;'","cspan":1,"rspan":1,"markup":[1,124]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: 'Ljava/util/List;->size()I'","cspan":1,"rspan":1,"markup":[1,94]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"This application executes a UNIX command containing this argument: '4'","cspan":1,"rspan":1,"markup":[0,70]},{"value":"34","cspan":1,"rspan":1,"markup":[1,2]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},null,null]},"options":{"table_caption":"Androwarn results of UNIX command execution on Android10 firmware.","table_label":"tab:AndrowarnUnixExamples"}}

==> assets/Tables/BuildBrandsModels <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Brands\n(ro.product.brand)","cspan":1,"rspan":1,"markup":[1,7,4,1,1,17]},{"value":"Manufacturers\n(ro.product.manufacturer)","cspan":1,"rspan":1,"markup":[1,39]},{"value":"Model\n(ro.product.model)","cspan":1,"rspan":1,"markup":[1,24]}],[{"value":"6","cspan":1,"rspan":1,"markup":[1,1]},{"value":"5","cspan":1,"rspan":1,"markup":[1,1]},{"value":"16","cspan":1,"rspan":1,"markup":[1,2]}],[{"value":"1","cspan":1,"rspan":1,"markup":[1,1]},{"value":"1","cspan":1,"rspan":1,"markup":[1,1]},{"value":"1","cspan":1,"rspan":1,"markup":[1,1]}],[{"value":"414","cspan":1,"rspan":1,"markup":[1,3]},{"value":"370","cspan":1,"rspan":1,"markup":[1,3]},{"value":"2004","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"193","cspan":1,"rspan":1,"markup":[1,3]},{"value":"186","cspan":1,"rspan":1,"markup":[1,3]},{"value":"760","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"134","cspan":1,"rspan":1,"markup":[1,3]},{"value":"120","cspan":1,"rspan":1,"markup":[1,3]},{"value":"543","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"81","cspan":1,"rspan":1,"markup":[1,2]},{"value":"79","cspan":1,"rspan":1,"markup":[1,2]},{"value":"407","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"21","cspan":1,"rspan":1,"markup":[1,2]},{"value":"24","cspan":1,"rspan":1,"markup":[1,2]},{"value":"186","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"10","cspan":1,"rspan":1,"markup":[1,2]},{"value":"9","cspan":1,"rspan":1,"markup":[1,1]},{"value":"101","cspan":1,"rspan":1,"markup":[1,3]}],[{"value":"-","cspan":1,"rspan":1,"markup":[1,1]},{"value":"-","cspan":1,"rspan":1,"markup":[1,1]},{"value":"-","cspan":1,"rspan":1,"markup":[1,1]}],[{"value":"2","cspan":1,"rspan":1,"markup":[1,1]},{"value":"2","cspan":1,"rspan":1,"markup":[1,1]},{"value":"2","cspan":1,"rspan":1,"markup":[1,1]}],[{"value":"862","cspan":1,"rspan":1,"markup":[1,3]},{"value":"796","cspan":1,"rspan":1,"markup":[1,3]},{"value":"420","cspan":1,"rspan":1,"markup":[1,3]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},null,null,{"style":{"fontWeight":"700","fontStyle":"normal","textDecoration":"","color":"","backgroundColor":""}},null]},"options":{"table_caption":"Overview of unique values in brand, manufacturer and model build properties by Android version.","table_label":"tab:FirmwareBrands"}}

==> assets/Tables/Certificates_AllVersionsTop <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"App developer\nand \nexample packagename","cspan":1,"rspan":1,"markup":[1,38]},{"value":"Certificate SHA1","cspan":1,"rspan":1,"markup":[1,16]},{"value":"Number of certificates\nin database","cspan":1,"rspan":1,"markup":[1,34]},{"value":"Percantage of total \napps in database \n(902'262)","cspan":1,"rspan":1,"markup":[1,48]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"Facebook \n(com.facebook.katana)","cspan":1,"rspan":1,"markup":[1,31]},{"value":"8A 3C 4B 26 2D 72 1A CD 49 A4 \nBF 97 D5 21 31 99 C8 6F A2 B9","cspan":1,"rspan":1,"markup":[1,60]},{"value":"2532","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.28%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},null]},"options":{"table_caption":"Top most certificates in our database.","table_label":"tab:Certificates_Top10"}}

==> assets/Tables/Certificates_Top10_8910 <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"App developer\nand \nexample packagename","cspan":1,"rspan":1,"markup":[1,38]},{"value":"Certificate SHA1","cspan":1,"rspan":1,"markup":[1,16]},{"value":"Number of certificates\nin database","cspan":1,"rspan":1,"markup":[1,34]},{"value":"Percantage of total \napps in database \n(902'262)","cspan":1,"rspan":1,"markup":[1,48]}],[{"value":"Android 10","cspan":4,"rspan":1,"markup":[3,10]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]}],[{"value":"Google Inc.\ncom.quicinc.cne.CNEService","cspan":1,"rspan":1,"markup":[1,38]},{"value":"E3 22 16 17 B1 D6  B5 10 DB 06 \n4E DB 38 15 02 BD FD 3B AC 47 ","cspan":1,"rspan":1,"markup":[1,62]},{"value":"1316","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.15%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.","cspan":1,"rspan":1,"markup":[1,11]},{"value":"38 91 8A 45 3D 07 19 93 54 F8 \nB1 9A F0 5E C6 56 2C ED 57 88 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1134","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.13%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\ncom.android.sharedstoragebackup","cspan":1,"rspan":1,"markup":[1,43]},{"value":"38 D8 1C FB 64 BD 5D 78 BA \nED 39 3C 25 E7 E9 2B 91 60 20 0E ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"869","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.10%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\nAndroid Easter Egg","cspan":1,"rspan":1,"markup":[1,30]},{"value":"69 25 F4 EE 29 7C 96 E8 30 5C \n59 EA 02 6B FA 74 A8 DC E1 91 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"869","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.10%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\ncom.android.vpndialogs","cspan":1,"rspan":1,"markup":[1,34]},{"value":"81 C2 B1 2C BA 14 66 FE CF \n45 29 BE 3F 08 14 B7 F5 0B 44 83 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"814","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.09%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\ncom.android.vpndialogs","cspan":1,"rspan":1,"markup":[1,34]},{"value":"81 90 2F C3 62 B6 A8 85 40 B2 \n7F 04 90 9C 2C 85 0A E8 46 85 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"814","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.09%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\ncom.quicinc.cne.CNEService","cspan":1,"rspan":1,"markup":[1,38]},{"value":"2A 5F D0 80 D1 5E D5 C6 91 36 \nB3 9A 9F 3E 64 C6 65 B9 91 A2 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"703","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.08%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\nandroid","cspan":1,"rspan":1,"markup":[1,19]},{"value":"D4 D3 D7 EF 20 B8 59 8A 43 71 \n49 9C AD 13 01 37 AA 30 FF 3B ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"703","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.08%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\nX Google enrollment","cspan":1,"rspan":1,"markup":[1,31]},{"value":"5F 3F 5A D9 2D 23 D6 40 2A 26 \n31 70 D8 7A 0D 8A 44 C5 90 AC ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"634","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.07%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\nDefault Print Service","cspan":1,"rspan":1,"markup":[1,33]},{"value":"70 62 71 04 12 02 F8 0C E2 AB\n09 DD 7C 22   95 9D 2D 92 DB 0C","cspan":1,"rspan":1,"markup":[1,61]},{"value":"634","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.07%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Android 9","cspan":4,"rspan":1,"markup":[3,9]},{"value":"C6 AE 38 2F FB 78 36 E3 4B 4F 49 9D 11 A4   1F E0 FE 00 3C B8 ","cspan":-1,"rspan":1,"markup":[1,62]},{"value":"384","cspan":-2,"rspan":1,"markup":[1,3]},{"value":"0.04","cspan":-3,"rspan":1,"markup":[1,4]}],[{"value":"Samsung\ncom.samsung.aasaservice","cspan":1,"rspan":1,"markup":[1,31]},{"value":"9C A5 17 0F 38 19 19 DF E0 44 \n6F CD AB 18 B1 9A 14 3B 31 63 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"21272","cspan":1,"rspan":1,"markup":[1,5]},{"value":"2.36%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.","cspan":1,"rspan":1,"markup":[1,11]},{"value":"38 91 8A 45 3D 07 19 93 54 F8 B1\n 9A F0 5E C6 56 2C ED 57 88 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"5577","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.62%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"InfinixMobility\nandroid","cspan":1,"rspan":1,"markup":[1,23]},{"value":"BF D5 79 80 68 4E B3 7C 5E 86 \nDA 0D D0 8A 9D DF E4 81 87 41 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1869","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.21%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Samsung (DMC)\ncom.android.dreams.basic","cspan":1,"rspan":1,"markup":[1,38]},{"value":"97 41 A0 F3 30 DC 2E 86 19 B7 \n6A 25 97 F3 08 C3 7D BE 30 A2 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1686","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.19%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Samsung Electronics Co. Ltd.\ncom.samsung.aasaservice","cspan":1,"rspan":1,"markup":[1,52]},{"value":"29 C6 47 CB CC 9A 5F BD 6C 0C\n 96 1E 05 71 2B D1 53 52 A1 F5 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1333","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.15%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\ncom.android.bluetooth","cspan":1,"rspan":1,"markup":[1,33]},{"value":"73 69 74 B3 71 23 FA 90 07 CF 05\n CD C1 FB   43 D9 15 91 76 22 ","cspan":1,"rspan":1,"markup":[1,63]},{"value":"1116","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.12%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\ncom.android.bluetooth","cspan":1,"rspan":1,"markup":[1,33]},{"value":"B8 41 56 6D C2 B4 69 F3 11 14\n BB 27 17 14   B5 DC A6 44 FD 80","cspan":1,"rspan":1,"markup":[1,62]},{"value":"1116","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.12%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google, Inc","cspan":1,"rspan":1,"markup":[1,11]},{"value":"24 BB 24 C0 5E 47 E0 AE FA 68\nA5 8A 76 61 79 D9 B6 13 A6 00 ","cspan":1,"rspan":1,"markup":[1,60]},{"value":"926","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.10%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\nandroid","cspan":1,"rspan":1,"markup":[1,19]},{"value":"D4 D3 D7 EF 20 B8 59 8A 43 71 \n49 9C AD 13 01 37 AA 30 FF 3B ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"919","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.10%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\ncom.quicinc.cne.CNEService","cspan":1,"rspan":1,"markup":[1,38]},{"value":"2A 5F D0 80 D1 5E D5 C6 91 36 \nB3 9A 9F 3E   64 C6 65 B9 91 A2 ","cspan":1,"rspan":1,"markup":[1,63]},{"value":"919","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0.10%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Android 8","cspan":4,"rspan":1,"markup":[2,9]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]}],[{"value":"Samsung\ncom.samsung.aasaservice","cspan":1,"rspan":1,"markup":[1,31]},{"value":"9C A5 17 0F 38 19 19 DF E0 44 6F \nCD AB 18 B1 9A 14 3B 31 63","cspan":1,"rspan":1,"markup":[1,60]},{"value":"19837","cspan":1,"rspan":1,"markup":[1,5]},{"value":"2.20%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.","cspan":1,"rspan":1,"markup":[1,11]},{"value":"38 91 8A 45 3D 07 19 93 54 F8 \nB1 9A F0 5E C6 56 2C ED 57 88 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"8731","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.97%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Transission\ncom.mediatek.batterywarning","cspan":1,"rspan":1,"markup":[1,39]},{"value":"BE 8C B9 F9 5B CB 5B FB 04 \n04 50 34 E5 18 26 34 A2 FC A1 FA ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"2421","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.27%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Samsung\ncom.samsung.aasaservice","cspan":1,"rspan":1,"markup":[1,31]},{"value":"29 C6 47 CB CC 9A 5F BD 6C \n0C 96 1E 05 71 2B D1 53 52 A1 F5 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1921","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.21%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google, Inc","cspan":1,"rspan":1,"markup":[1,11]},{"value":"24 BB 24 C0 5E 47 E0 AE FA 68 \nA5 8A 76 61 79 D9 B6 13 A6 00 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1852","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.21%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Samsung Corporation (DMC)","cspan":1,"rspan":1,"markup":[1,25]},{"value":"97 41 A0 F3 30 DC 2E 86 19 B7 \n6A 25 97 F3 08 C3 7D BE 30 A2 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1720","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.19%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Zhantang\ncom.sprd.engineermode","cspan":1,"rspan":1,"markup":[1,30]},{"value":"F1 A5 4A 3F 02 4A 8D 1B 74 D1 \nFF 1F 74 D3 BE 66 ED 79 31 2E ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1478","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.16%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Google Inc.\ncom.android.egg","cspan":1,"rspan":1,"markup":[1,27]},{"value":"69 25 F4 EE 29 7C 96 E8 30 5C \n59 EA 02 6B FA 74 A8 DC E1 91 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1407","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.16%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Tecno\n","cspan":1,"rspan":1,"markup":[1,6]},{"value":"48 19 D1 56 9B D0 64 AD 33 94 \n61 73 79 32 FB 76 1C 1B E1 77 ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1323","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.15%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"Lava\ncom.adups.fota","cspan":1,"rspan":1,"markup":[1,19]},{"value":"FB 01 33 26 78 40 78 4C A3 00 \n9E 26 F2 69 F7 43 2C 09 19 EC ","cspan":1,"rspan":1,"markup":[1,61]},{"value":"1184","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.13%","cspan":1,"rspan":1,"markup":[1,5]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":""}},{"style":{"fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},null,null]},"options":{"table_caption":"Top ten most used certificates for Android 8, 9, and 10 in our database.","table_label":"tab:Certificates_Top5perVersion"}}

==> assets/Tables/Certificates_Top5PerVersion <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"italic":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"App developer\nand \nexample packagename","cspan":1,"rspan":1,"markup":[1,38]},{"value":"Certificate SHA1","cspan":1,"rspan":1,"markup":[1,16]},{"value":"Number of certificates\nin database","cspan":1,"rspan":1,"markup":[1,34]},{"value":"Percantage of total \napps in database \n(902'262)","cspan":1,"rspan":1,"markup":[1,48]}],[{"value":"Android 10","cspan":4,"rspan":1,"markup":[3,10]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]}],[{"value":"Facebook \n(com.facebook.katana)","cspan":1,"rspan":1,"markup":[1,31]},{"value":"8A 3C 4B 26 2D 72 1A CD 49 A4 \nBF 97 D5 21 31 99 C8 6F A2 B9","cspan":1,"rspan":1,"markup":[1,60]},{"value":"2532","cspan":1,"rspan":1,"markup":[1,4]},{"value":"0.28%","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"Android 9","cspan":4,"rspan":1,"markup":[3,9]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"Android 8","cspan":4,"rspan":1,"markup":[2,9]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"","cspan":-2,"rspan":1,"markup":[]},{"value":"","cspan":-3,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":""}},{"style":{"fontStyle":"","textDecoration":"","color":"","backgroundColor":""}}]},"options":{"table_caption":"Top five most certificates in our database for Android 8, 9, and 10.","table_label":"tab:Certificates_Top5perVersion"}}

==> assets/Tables/Certificates_uniques <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Android \nVersion","cspan":1,"rspan":1,"markup":[2,16]},{"value":"Total number\nof certificates\nextracted","cspan":1,"rspan":1,"markup":[1,38]},{"value":"Number of \nunique\ncertificates","cspan":1,"rspan":1,"markup":[2,30]},{"value":"Ratio unique \npackagename to \nunique certificate","cspan":1,"rspan":1,"markup":[2,48]}],[{"value":"8","cspan":1,"rspan":1,"markup":[2,1]},{"value":"72'076","cspan":1,"rspan":1,"markup":[2,6]},{"value":"447","cspan":1,"rspan":1,"markup":[2,3]},{"value":"1'991/447","cspan":1,"rspan":1,"markup":[2,9]}],[{"value":"9","cspan":1,"rspan":1,"markup":[2,1]},{"value":"55'291","cspan":1,"rspan":1,"markup":[2,6]},{"value":"320","cspan":1,"rspan":1,"markup":[2,3]},{"value":"1'375/320","cspan":1,"rspan":1,"markup":[2,9]}],[{"value":"10","cspan":1,"rspan":1,"markup":[2,2]},{"value":"15'130","cspan":1,"rspan":1,"markup":[2,6]},{"value":"92","cspan":1,"rspan":1,"markup":[2,2]},{"value":"242/92","cspan":1,"rspan":1,"markup":[2,6]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},null]},"options":{"table_caption":"Number of unique certificates in our database.","table_label":"tab:Certificates_Unique"}}

==> assets/Tables/Literature_Search_ltx <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Title","cspan":1,"rspan":1,"markup":[2,5]},{"value":"Year","cspan":1,"rspan":1,"markup":[2,4]},{"value":"Relvant","cspan":1,"rspan":1,"markup":[2,7]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8984540/}{A   ransomware detection method using fuzzy hashing for mitigating the risk of   occlusion of information systems}","cspan":1,"rspan":1,"markup":[1,176]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8858803/}{Cyberthreat   Hunting-Part 1: triaging ransomware using fuzzy hashing, import hashing and   YARA rules}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8858825/}{Cyberthreat   hunting-part 2: Tracking ransomware threat actors using fuzzy hashing and   fuzzy c-means clustering}","cspan":1,"rspan":1,"markup":[1,177]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9177636/}{Fuzzy-Import   Hashing: A malware analysis approach}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9308189/}{Fuzzy   hashing aided enhanced YARA rules for malware triaging}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9003148/}{Lockout-Tagout   Ransomware: A detection method for ransomware using fuzzy hashing and   clustering}","cspan":1,"rspan":1,"markup":[1,162]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9002773/}{Augmented   YARA rules fused with fuzzy hashing in ransomware triaging}","cspan":1,"rspan":1,"markup":[1,133]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/cset15/workshop-program/presentation/li}{Experimental   study of fuzzy hashing in malware clustering analysis}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7575849/}{Detection   of malicious portable executables using evidence combinational theory with   fuzzy hashing}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://commons.erau.edu/adfsl/2012/wednesday/15/}{A   fuzzy hashing approach based on random sequences and hamming distance}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1742287613000789}{F2S2:   Fast forensic similarity search through indexing piecewise hash signatures}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://core.ac.uk/download/pdf/46911337.pdf}{Security   Aspects of Fuzzy Hashing}","cspan":1,"rspan":1,"markup":[1,88]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7847157/}{Forensic   malware analysis: The value of fuzzy hashing algorithms in identifying   similarities}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://digital.csic.es/handle/10261/135088}{A   new edit distance for fuzzy hashing applications}","cspan":1,"rspan":1,"markup":[1,104]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-49445-6_15}{Malware   characterization using windows API call sequences}","cspan":1,"rspan":1,"markup":[1,130]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6754635/}{TLSH--a   locality sensitive hash}","cspan":1,"rspan":1,"markup":[1,96]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.koreascience.or.kr/article/JAKO201208138130922.page}{Research   on the classification model of similarity malware using fuzzy hash}","cspan":1,"rspan":1,"markup":[1,149]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-642-19931-8_15}{Web   document duplicate detection using fuzzy hashing}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6754635/}{TLSH--a   locality sensitive hash}","cspan":1,"rspan":1,"markup":[1,96]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3176258.3176306}{Beyond   precision and recall: understanding uses (and misuses) of similarity hashes   in binary analysis}","cspan":1,"rspan":1,"markup":[1,164]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7847157/}{Forensic   malware analysis: The value of fuzzy hashing algorithms in identifying   similarities}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3077286.3077289}{A   comparison of fuzzy hashes: evaluation, guidelines, and future suggestions}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-662-45670-5_19}{Using   randomization to attack similarity digests}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-04503-6_19}{Dynamic   Whitelisting Using Locality Sensitive Hashing}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-99277-8_12}{Hashing   Incomplete and Unordered Network Streams}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7371622/}{Document   Copy Detection Using the Improved Fuzzy Hashing}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9191381/}{Hac-t   and fast search for similarity in security}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9280546/}{Scalable   Malware Clustering using Multi-Stage Tree Parallelization}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.mdpi.com/2076-3417/10/15/5173}{Combined   kNN Classification and hierarchical similarity hash for fast malware   detection}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9110432/}{Clustering   IoT Malware based on Binary Similarity}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://webdiis.unizar.es/~ricardo/files/TFGs/FuzzyHashingProcesos.pdf}{Evaluación   de algoritmos de fuzzy hashing para similitud entre procesos}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.mesalab.cn/managercode/achievements/%E8%AE%BA%E6%96%87%EF%BC%9ASFH%20Hashing%20Unordered%20and%20Incomplete%20network%20traffic%20on%20the%20fly.pdf}{SFH:   Hashing Unordered and Incomplete Network Streams on the Fly}","cspan":2,"rspan":1,"markup":[1,235]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8658199/}{An   entropy-based solution for identifying android packers}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://mountainscholar.org/handle/11124/173074}{Similarity   hashing of malware on IoT devices}","cspan":1,"rspan":1,"markup":[1,102]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1901.02438}{Using   fuzzy bits and neural networks to partially invert few rounds of some   cryptographic hash functions}","cspan":1,"rspan":1,"markup":[1,149]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://commons.erau.edu/cgi/viewcontent.cgi?article=1379&context=jdfsl}{Bytewise   approximate matching: the good, the bad, and the unknown}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6754635/}{TLSH--a   locality sensitive hash}","cspan":1,"rspan":1,"markup":[1,96]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3176258.3176306}{Beyond   precision and recall: understanding uses (and misuses) of similarity hashes   in binary analysis}","cspan":1,"rspan":1,"markup":[1,164]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7847157/}{Forensic   malware analysis: The value of fuzzy hashing algorithms in identifying   similarities}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3077286.3077289}{A   comparison of fuzzy hashes: evaluation, guidelines, and future suggestions}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-662-45670-5_19}{Using   randomization to attack similarity digests}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-04503-6_19}{Dynamic   Whitelisting Using Locality Sensitive Hashing}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-99277-8_12}{Hashing   Incomplete and Unordered Network Streams}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7371622/}{Document   Copy Detection Using the Improved Fuzzy Hashing}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9191381/}{Hac-t   and fast search for similarity in security}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9280546/}{Scalable   Malware Clustering using Multi-Stage Tree Parallelization}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.mdpi.com/2076-3417/10/15/5173}{Combined   kNN Classification and hierarchical similarity hash for fast malware   detection}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9110432/}{Clustering   IoT Malware based on Binary Similarity}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://webdiis.unizar.es/~ricardo/files/TFGs/FuzzyHashingProcesos.pdf}{Evaluación   de algoritmos de fuzzy hashing para similitud entre procesos}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.mesalab.cn/managercode/achievements/%E8%AE%BA%E6%96%87%EF%BC%9ASFH%20Hashing%20Unordered%20and%20Incomplete%20network%20traffic%20on%20the%20fly.pdf}{SFH:   Hashing Unordered and Incomplete Network Streams on the Fly}","cspan":2,"rspan":1,"markup":[1,235]},{"value":"","cspan":-1,"rspan":1,"markup":[]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8658199/}{An   entropy-based solution for identifying android packers}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://mountainscholar.org/handle/11124/173074}{Similarity   hashing of malware on IoT devices}","cspan":1,"rspan":1,"markup":[1,102]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1901.02438}{Using   fuzzy bits and neural networks to partially invert few rounds of some   cryptographic hash functions}","cspan":1,"rspan":1,"markup":[1,149]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://commons.erau.edu/cgi/viewcontent.cgi?article=1379&context=jdfsl}{Bytewise   approximate matching: the good, the bad, and the unknown}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1742287617302566}{Lempel-Ziv   Jaccard Distance, an effective alternative to ssdeep and sdhash}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://content.sciendo.com/view/journals/slgr/56/1/article-p45.xml}{Application   of Normalized Compression Distance and Lempel-Ziv Jaccard Distance in   Micro-electrode Signal Stream Classification for the Surgical Treatment of …}","cspan":1,"rspan":1,"markup":[1,238]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3128572.3140446}{Malware   classification and class imbalance via stochastic hashed LZJD}","cspan":1,"rspan":1,"markup":[1,130]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://mountainscholar.org/handle/11124/173074}{Similarity   hashing of malware on IoT devices}","cspan":1,"rspan":1,"markup":[1,102]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://itiis.org/journals/tiis/digital-library/manuscript/file/23099/TIIS%20Vol%2013,%20No%2012-19.pdf}{Fast   k-NN based Malware Analysis in a Massive Malware Environment.}","cspan":1,"rspan":1,"markup":[1,179]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9191381/}{Hac-t   and fast search for similarity in security}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1910.07283}{Fishdbc:   Flexible, incremental, scalable, hierarchical density-based clustering for   arbitrary data and distance}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.mdpi.com/2227-7390/8/4/503}{An   Improved Bytewise Approximate Matching Algorithm Suitable for Files of   Dissimilar Sizes}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8514832/}{mrsh-mem:   Approximate matching on raw memory dumps}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/content/pdf/10.1007/978-3-030-39250-5.pdf}{Data   Science: New Issues, Challenges and Applications}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167404818303808}{Survey   of machine learning techniques for malware analysis}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.mdpi.com/1099-4300/21/12/1196}{A   Survey on Using Kolmogorov Complexity in Cybersecurity}","cspan":1,"rspan":1,"markup":[1,108]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8988556/}{A   Mechanism for Copyright Protection under Information-Centric Networking}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.crysys.hu/publications/files/setit/thesis_bme_Bak19bsc.pdf}{Clustering   IoT Malware Samples based on Binary Similarity}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/5766764/}{Understanding   plagiarism linguistic patterns, textual features, and detection methods}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://arxiv.org/abs/2006.09271}{A   Survey of Machine Learning Methods and Challenges for Windows Malware   Classification}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://spectrum.library.concordia.ca/978935/}{a   framework for automated similarity analysis of malware}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8858803/}{Cyberthreat   Hunting-Part 1: triaging ransomware using fuzzy hashing, import hashing and   YARA rules}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8984540/}{A   ransomware detection method using fuzzy hashing for mitigating the risk of   occlusion of information systems}","cspan":1,"rspan":1,"markup":[1,176]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9177636/}{Fuzzy-Import   Hashing: A malware analysis approach}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9002773/}{Augmented   YARA rules fused with fuzzy hashing in ransomware triaging}","cspan":1,"rspan":1,"markup":[1,133]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/cset15/workshop-program/presentation/li}{Experimental   study of fuzzy hashing in malware clustering analysis}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://commons.erau.edu/adfsl/2012/wednesday/15/}{A   fuzzy hashing approach based on random sequences and hamming distance}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8858825/}{Cyberthreat   hunting-part 2: Tracking ransomware threat actors using fuzzy hashing and   fuzzy c-means clustering}","cspan":1,"rspan":1,"markup":[1,177]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9003148/}{Lockout-Tagout   Ransomware: A detection method for ransomware using fuzzy hashing and   clustering}","cspan":1,"rspan":1,"markup":[1,162]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9308189/}{Fuzzy   hashing aided enhanced YARA rules for malware triaging}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ntnuopen.ntnu.no/ntnu-xmlui/bitstream/handle/11250/144008/KPAstebol.pdf?sequence=1}{mvHash:   a new approach for fuzzy hashing}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7847157/}{Forensic   malware analysis: The value of fuzzy hashing algorithms in identifying   similarities}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6754635/}{TLSH--a   locality sensitive hash}","cspan":1,"rspan":1,"markup":[1,96]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://www.dasec.h-da.de/wp-content/uploads/2012/08/2012_08_Breitinger_NeSeFo.pdf}{Security   and implementation analysis of the similarity digest sdhash}","cspan":1,"rspan":1,"markup":[1,160]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1742287613000789}{F2S2:   Fast forensic similarity search through indexing piecewise hash signatures}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6320445/}{Properties   of a similarity preserving hash function and their realization in sdhash}","cspan":1,"rspan":1,"markup":[1,148]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7575849/}{Detection   of malicious portable executables using evidence combinational theory with   fuzzy hashing}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3077286.3077289}{A   comparison of fuzzy hashes: evaluation, guidelines, and future suggestions}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1742287617302566}{Lempel-Ziv   Jaccard Distance, an effective alternative to ssdeep and sdhash}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://kilthub.cmu.edu/articles/journal_contribution/Results_of_SEI_Line-Funded_Exploratory_New_Starts_Projects/6583433/files/12070334.pdf#page=9}{2   Fuzzy Hashing Techniques in Applied Malware Analysis}","cspan":1,"rspan":1,"markup":[1,211]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/cset15/workshop-program/presentation/li}{Experimental   study of fuzzy hashing in malware clustering analysis}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9002773/}{Augmented   YARA rules fused with fuzzy hashing in ransomware triaging}","cspan":1,"rspan":1,"markup":[1,133]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8858803/}{Cyberthreat   Hunting-Part 1: triaging ransomware using fuzzy hashing, import hashing and   YARA rules}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9177636/}{Fuzzy-Import   Hashing: A malware analysis approach}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9056506/}{Deep   fuzzy hashing network for efficient image retrieval}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://commons.erau.edu/adfsl/2012/wednesday/15/}{A   fuzzy hashing approach based on random sequences and hamming distance}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9308189/}{Fuzzy   hashing aided enhanced YARA rules for malware triaging}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8858825/}{Cyberthreat   hunting-part 2: Tracking ransomware threat actors using fuzzy hashing and   fuzzy c-means clustering}","cspan":1,"rspan":1,"markup":[1,177]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9177856/}{Embedding   fuzzy rules with YARA rules for performance optimisation of malware analysis}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.irojournals.com/itdw/V2/I3/03.pdf}{A   Novel Information retrieval system for distributed cloud using Hybrid Deep   Fuzzy Hashing Algorithm}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-642-35515-8_12}{Performance   issues about context-triggered piecewise hashing}","cspan":1,"rspan":1,"markup":[1,133]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2093698.2093722}{On   fuzzy syndrome hashing with LDPC coding}","cspan":1,"rspan":1,"markup":[1,103]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://kilthub.cmu.edu/articles/journal_contribution/Results_of_SEI_Line-Funded_Exploratory_New_Starts_Projects/6583433/files/12070334.pdf#page=9}{2   Fuzzy Hashing Techniques in Applied Malware Analysis}","cspan":1,"rspan":1,"markup":[1,211]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.igi-global.com/article/scaling-up-software-birthmarks-using-fuzzy-hashing/182539}{Scaling   up software birthmarks using fuzzy hashing}","cspan":1,"rspan":1,"markup":[1,153]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7550868/}{A   fuzzy hashing technique for large scale software birthmarks}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ntnuopen.ntnu.no/ntnu-xmlui/bitstream/handle/11250/144008/KPAstebol.pdf?sequence=1}{mvHash:   a new approach for fuzzy hashing}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/cset15/workshop-program/presentation/li}{Experimental   study of fuzzy hashing in malware clustering analysis}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9003148/}{Lockout-Tagout   Ransomware: A detection method for ransomware using fuzzy hashing and   clustering}","cspan":1,"rspan":1,"markup":[1,162]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8858825/}{Cyberthreat   hunting-part 2: Tracking ransomware threat actors using fuzzy hashing and   fuzzy c-means clustering}","cspan":1,"rspan":1,"markup":[1,177]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8984540/}{A   ransomware detection method using fuzzy hashing for mitigating the risk of   occlusion of information systems}","cspan":1,"rspan":1,"markup":[1,176]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2684793.2684803}{Clustering   spam campaigns with fuzzy hashing}","cspan":1,"rspan":1,"markup":[1,105]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9177636/}{Fuzzy-Import   Hashing: A malware analysis approach}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8858803/}{Cyberthreat   Hunting-Part 1: triaging ransomware using fuzzy hashing, import hashing and   YARA rules}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9002773/}{Augmented   YARA rules fused with fuzzy hashing in ransomware triaging}","cspan":1,"rspan":1,"markup":[1,133]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7575849/}{Detection   of malicious portable executables using evidence combinational theory with   fuzzy hashing}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9308189/}{Fuzzy   hashing aided enhanced YARA rules for malware triaging}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://search.proquest.com/openview/8eb7000746ead07670846cb651554f36/1?pq-origsite=gscholar&cbl=1976342}{Evaluation   on malware classification by combining traffic analysis and fuzzy hashing of   malware binary}","cspan":1,"rspan":1,"markup":[1,219]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.irojournals.com/itdw/V2/I3/03.pdf}{A   Novel Information retrieval system for distributed cloud using Hybrid Deep   Fuzzy Hashing Algorithm}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6031914/}{Multiple   kernel fuzzy clustering}","cspan":1,"rspan":1,"markup":[1,97]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9177856/}{Embedding   fuzzy rules with YARA rules for performance optimisation of malware analysis}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3041008.3041010}{Emulator   vs real phone: Android malware detection using machine learning}","cspan":1,"rspan":1,"markup":[1,133]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590325}{Evading   android runtime analysis via sandbox detection}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2664243.2664250}{Morpheus:   automatically generating heuristics to detect android emulators}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2799979.2800004}{A   robust dynamic analysis system preventing SandBox detection by Android   malware}","cspan":1,"rspan":1,"markup":[1,143]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6583806/}{Applying   machine learning classifiers to dynamic android malware detection at scale}","cspan":1,"rspan":1,"markup":[1,148]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7389671/}{A   study of android malware detection technology evolution}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2592791.2592796}{Rage   against the virtual machine: hindering dynamic analysis of android malware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.koreascience.or.kr/article/ArticleFullRecord.jsp?cn=JBBHCB_2015_v25n5_1067}{A   Study on android emulator detection for mobile game security}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2875475.2875487}{Evaluation   of android malware detection based on system calls}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6982893/}{Malware   detection using network traffic analysis in android based mobile devices}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.cs.utah.edu/docs/techreports/2015/pdf/UUCS-15-003.pdf}{Android   malware detection based on system calls}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3386415.3387091}{Out-of-Domain   Characteristic Based Hierarchical Emulator Detection for Mobile}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S2352340918315774}{Data   on vulnerability detection in android}","cspan":1,"rspan":1,"markup":[1,120]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1877050916001071}{Anti-Hijack:   Runtime detection of malware initiated hijacking in android}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2940343.2940348}{CREDROID:   Android malware detection by network traffic analysis}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7814490/}{Deep4maldroid:   A deep learning framework for android malware detection based on linux kernel   system call graphs}","cspan":1,"rspan":1,"markup":[1,178]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.mdpi.com/558048}{AndroShield:   automated android applications vulnerability detection, a hybrid static and   dynamic analysis approach}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2480362.2480701}{Mobile-sandbox:   having a deeper look into android applications}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2808117.2808126}{Android   rooting: Methods, detection, and evasion}","cspan":1,"rspan":1,"markup":[1,109]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://rp.delaat.net/2015-2016/p51/report.pdf}{Jailbreak/root   detection evasion study on iOS and Android}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2810362.2810364}{All   your root checks are belong to us: The sad state of root detection}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2307636.2307663}{Riskranker:   scalable and accurate zero-day android malware detection}","cspan":1,"rspan":1,"markup":[1,129]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-68542-7_69}{System   log-based android root state detection}","cspan":1,"rspan":1,"markup":[1,118]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2810103.2813714}{Android   root and its providers: A double-edged sword}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6128277/}{Kernel-based   behavior analysis for android malware detection}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/2012.01812}{On   Root Detection Strategies for Android Devices}","cspan":1,"rspan":1,"markup":[1,91]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-04283-1_6}{Droidapiminer:   Mining api-level features for robust malware detection in android}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s10916-018-0966-x}{Root   exploit detection and features optimization: mobile device and blockchain   based medical data management}","cspan":1,"rspan":1,"markup":[1,180]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8399047/}{User   conventional root detection for indoor mall}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2557547.2557563}{PREC:   practical root exploit containment for android devices}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.researchgate.net/profile/Hugo_Gascon/publication/264785935_DREBIN_Effective_and_Explainable_Detection_of_Android_Malware_in_Your_Pocket/links/53efd0020cf26b9b7dcdf395.pdf}{Drebin:   Effective and explainable detection of android malware in your pocket.}","cspan":1,"rspan":1,"markup":[1,271]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity17/technical-sessions/presentation/gasparis}{Detecting   android root exploits by learning from root providers}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8074847/}{Malware   detection in android based on dynamic analysis}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2435349.2435377}{Fast,   scalable detection of piggybacked mobile applications}","cspan":1,"rspan":1,"markup":[1,120]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6182000/}{Rooting   attack detection method on the Android-based smart phone}","cspan":1,"rspan":1,"markup":[1,129]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6735264/}{Machine   learning for android malware detection using permission and api calls}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7972730/}{Who   changed you? Obfuscator identification for Android}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3129676.3129708}{An   anti-reverse engineering technique using native code and obfuscator-llvm for   android applications}","cspan":1,"rspan":1,"markup":[1,163]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1907.06828}{Automated   deobfuscation of Android native binary code}","cspan":1,"rspan":1,"markup":[1,96]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-03783-7_10}{Efficient   code obfuscation for Android}","cspan":1,"rspan":1,"markup":[1,111]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2976749.2978333}{Reliable   third-party library detection in android and its security applications}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://papers.ssrn.com/sol3/papers.cfm?abstract_id=3511052}{TargO:   A Targeted Obfuscator for Android Applications}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8802781/}{Deobfuscating   Android native binary code}","cspan":1,"rspan":1,"markup":[1,105]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2843859.2843866}{Enriching   reverse engineering through visual exploration of Android binaries}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6149548/}{Android:   Static analysis using similarity distance}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://net.cs.uni-bonn.de/fileadmin/user_upload/plohmann/2012-Schulz-Code_Protection_in_Android.pdf}{Code   protection in android}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167404816300529}{Control   flow obfuscation for android applications}","cspan":1,"rspan":1,"markup":[1,127]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s11416-016-0282-2}{Testing   android malware detectors against code obfuscation: a systematization of   knowledge and unified methodology}","cspan":1,"rspan":1,"markup":[1,186]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2751323.2751330}{Exploring   reverse engineering symptoms in Android apps}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://media.blackhat.com/bh-ad-11/Desnos/bh-ad-11-DesnosGueguen-Andriod-Reversing_to_Decompilation_WP.pdf}{Android:   From reversing to decompilation}","cspan":1,"rspan":1,"markup":[1,157]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-01701-9_10}{Understanding   android obfuscation techniques: A large-scale investigation in the wild}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2635868.2635869}{Apposcopy:   Semantics-based detection of android malware through static analysis}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s10766-018-0609-3}{Prodact:   Prefetch-obfuscator to defend against cache timing channels}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=WAaJEN4ZI-QC&oi=fnd&pg=PR1&dq=android+obfuscator&ots=zGuGGaOTpx&sig=L9ZK7yWHaoPYijyPys3DNueNMHI}{Decompiling   android}","cspan":1,"rspan":1,"markup":[1,169]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2976749.2978422}{Statistical   deobfuscation of android applications}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3099012.3099020}{Anti-proguard:   Towards automated deobfuscation of android apps}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1907.06828}{Automated   deobfuscation of Android native binary code}","cspan":1,"rspan":1,"markup":[1,96]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://tests.virusbtn.com/uploads/pdf/magazine/2018/VB2018-Moses-Mordekhay.pdf}{Android   app deobfuscation using static-dynamic cooperation}","cspan":1,"rspan":1,"markup":[1,148]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.koreascience.or.kr/article/JAKO201533678768418.page}{A   study on deobfuscation method of Android and implementation of automatic   analysis tool}","cspan":1,"rspan":1,"markup":[1,164]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3196398.3196433}{Leveraging   historical versions of Android apps for efficient and precise taint analysis}","cspan":1,"rspan":1,"markup":[1,148]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8802781/}{Deobfuscating   Android native binary code}","cspan":1,"rspan":1,"markup":[1,105]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity18/presentation/wong}{Tackling   runtime-based obfuscation in Android with TIRO}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://jbremer.org/wp-posts/athcon.pdf}{Automated   analysis and deobfuscation of android apps & malware}","cspan":1,"rspan":1,"markup":[1,111]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167404820300936}{Compile-time   code virtualization for android applications}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-03783-7_10}{Efficient   code obfuscation for Android}","cspan":1,"rspan":1,"markup":[1,111]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3289239.3289243}{Dose:   Deobfuscation based on semantic equivalence}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7985674/}{Libd:   Scalable and precise third-party library detection in android markets}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://manuscriptlink-society-file.s3.amazonaws.com/kism/conference/sma2020/presentation/SMA-2020_paper_75.pdf}{Reversing   Obfuscated Control Flow Structures in Android Apps using ReDex Optimizer}","cspan":1,"rspan":1,"markup":[1,203]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1574013721000058}{A   survey of android application and malware hardening}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2021","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.ndss-symposium.org/wp-content/uploads/2017/09/harvesting-runtime-values-android-applications-feature-anti-analysis-techniques.pdf}{Harvesting   Runtime Values in Android Applications That Feature Anti-Analysis   Techniques.}","cspan":1,"rspan":1,"markup":[1,242]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://isyou.info/inpra/papers/inpra-v4n2-01.pdf}{String   deobfuscation scheme based on dynamic code extraction for mobile malwares}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.inderscienceonline.com/doi/abs/10.1504/IJAHUC.2019.100730}{Automatic   string deobfuscation scheme for mobile applications based on platform-level   code extraction}","cspan":1,"rspan":1,"markup":[1,183]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2999572.2999596}{Enabling   automatic protocol behavior analysis for android applications}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-24177-7_15}{Dexhunter:   toward extracting hidden code from packed android applications}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.cs.ucr.edu/~heng/pubs/DroidUnpack_ndss18.pdf}{Things   You May Not Know About Android (Un) Packers: A Systematic Study based on   Whole-System Emulation.}","cspan":1,"rspan":1,"markup":[1,172]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-26362-5_17}{Appspear:   Bytecode decrypting and dex reassembling for packed android malware}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www2.virusbulletin.com/uploads/pdf/conference/vb2014/VB2014-Yu.pdf}{Android   packers: facing the challenges, building solutions}","cspan":1,"rspan":1,"markup":[1,143]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7787078/}{Automated   detection and classification for packed android applications}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7985676/}{Adaptive   unpacking of Android apps}","cspan":1,"rspan":1,"markup":[1,99]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9144572/}{DroidPDF:   The Obfuscation Resilient Packer Detection Framework for Android Apps}","cspan":1,"rspan":1,"markup":[1,144]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8490853/}{DexX:   a double layer unpacking framework for Android}","cspan":1,"rspan":1,"markup":[1,117]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0164121218300311}{AppSpear:   automating the hidden-code extraction and reassembling of packed android   malware}","cspan":1,"rspan":1,"markup":[1,170]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://net.cs.uni-bonn.de/fileadmin/user_upload/plohmann/2012-Schulz-Code_Protection_in_Android.pdf}{Code   protection in android}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9098088/}{PackerGrind:   An Adaptive Unpacking System for Android Apps}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8658199/}{An   entropy-based solution for identifying android packers}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167404820300936}{Compile-time   code virtualization for android applications}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://surface.syr.edu/etd/498/}{Automated   code extraction from packed android applications.}","cspan":1,"rspan":1,"markup":[1,102]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8812043/}{Storydroid:   Automated generation of storyboard for Android apps}","cspan":1,"rspan":1,"markup":[1,128]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7961511/}{RepDroid:   an automated tool for Android application repackaging detection}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7972730/}{Who   changed you? Obfuscator identification for Android}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-18681-8_24}{Uncovering   self code modification in android}","cspan":1,"rspan":1,"markup":[1,117]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2523514.2523539}{AndroSimilar:   robust statistical feature signature for Android malware detection}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-03783-7_10}{Efficient   code obfuscation for Android}","cspan":1,"rspan":1,"markup":[1,111]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7985676/}{Adaptive   unpacking of Android apps}","cspan":1,"rspan":1,"markup":[1,99]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8490853/}{DexX:   a double layer unpacking framework for Android}","cspan":1,"rspan":1,"markup":[1,117]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-24177-7_15}{Dexhunter:   toward extracting hidden code from packed android applications}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.cs.ucr.edu/~heng/pubs/DroidUnpack_ndss18.pdf}{Things   You May Not Know About Android (Un) Packers: A Systematic Study based on   Whole-System Emulation.}","cspan":1,"rspan":1,"markup":[1,172]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9098088/}{PackerGrind:   An Adaptive Unpacking System for Android Apps}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0164121218300311}{AppSpear:   automating the hidden-code extraction and reassembling of packed android   malware}","cspan":1,"rspan":1,"markup":[1,170]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167404820300936}{Compile-time   code virtualization for android applications}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www8.virusbtn.com/uploads/pdf/magazine/2018/VB2018-Stone.pdf}{UNPACKING   THE PACKED UNPACKER: REVERSING AN ANDROID ANTI-ANALYSIS NATIVE LIBRARY}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity18/presentation/wong}{Tackling   runtime-based obfuscation in Android with TIRO}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://hitcon.org/2015/ENT/PDF/The%20Terminator%20to%20Android%20Hardening%20Services_Yueqian%20Zhang,%20Xiapu%20Luo,%20Haoyang%20Yin.pdf}{The   terminator to Android hardening services}","cspan":1,"rspan":1,"markup":[1,192]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8293854/}{Android   malware familial classification and representative sample selection via   frequent subgraph analysis}","cspan":1,"rspan":1,"markup":[1,173]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-26362-5_17}{Appspear:   Bytecode decrypting and dex reassembling for packed android malware}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://net.cs.uni-bonn.de/fileadmin/user_upload/plohmann/2012-Schulz-Code_Protection_in_Android.pdf}{Code   protection in android}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8812083/}{Graph   embedding based familial analysis of android malware using unsupervised   learning}","cspan":1,"rspan":1,"markup":[1,153]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2557547.2557558}{Divilar:   Diversifying intermediate language for anti-repackaging on android platform}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s42452-019-1124-x}{The   Android malware detection systems between hope and reality}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-93411-2_4}{Honey,   i shrunk your app security: The state of android app hardening}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8770262/}{Ctdroid:   leveraging a corpus of technical blogs for android malware analysis}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-24018-3_12}{How   current android malware seeks to evade automated code analysis}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2897845.2897914}{revdroid:   Code analysis of the side effects after dynamic permission revocation of   android apps}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0045790617303087}{Machine   learning aided Android malware classification}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/2003.12730}{How   and Why did developers migrate Android Applications from Java to Kotlin? A   study based on code analysis and interviews with developers}","cspan":1,"rspan":1,"markup":[1,183]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8094472/}{DroidFax:   A toolkit for systematic characterization of Android applications}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2699026.2699105}{Stadyna:   Addressing the problem of dynamic code updates in the security analysis of   android applications}","cspan":1,"rspan":1,"markup":[1,167]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1410.7749}{Enter   sandbox: Android sandbox comparison}","cspan":1,"rspan":1,"markup":[1,83]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-01701-9_10}{Understanding   android obfuscation techniques: A large-scale investigation in the wild}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.rasthofer.info/publications/paper/TR2015-Harvester.pdf}{Harvesting   runtime data in android applications for identifying malware and enhancing   code analysis}","cspan":1,"rspan":1,"markup":[1,178]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7077314/}{Android   malware classification using static code analysis and Apriori algorithm   improved with particle swarm optimization}","cspan":1,"rspan":1,"markup":[1,188]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6258449/}{Analysis   of android applications' permissions}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://net.cs.uni-bonn.de/fileadmin/user_upload/plohmann/2012-Schulz-Code_Protection_in_Android.pdf}{Code   protection in android}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0950584912001012}{Static   analysis of Android programs}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7972730/}{Who   changed you? Obfuscator identification for Android}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-642-27207-3_33}{Mobile   application compatibility test system design for android fragmentation}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7019227/}{Detecting   software vulnerabilities in android using static analysis}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2382196.2382205}{Why   Eve and Mallory love Android: An analysis of Android SSL (in) security}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7180133/}{A   dataset of open-source android applications}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2536853.2536881}{Droidfuzzer:   Fuzzing the android apps with intent-filter tag}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7985671/}{Making   malory behave maliciously: Targeted fuzzing of android execution   environments}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3407023.3407052}{Template-based   Android inter process communication fuzzing}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/liu}{FANS:   Fuzzing Android Native System Services via Automated Interface Analysis}","cspan":1,"rspan":1,"markup":[1,155]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://web.cse.ohio-state.edu/~zhao.2708/assets/ndss18/NDSS18.pdf}{IoTFuzzer:   Discovering Memory Corruptions in IoT Through App-based Fuzzing.}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3386901.3388916}{Vulcan:   Lessons on reliability of wearables through state-aware fuzzing}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2639108.2639131}{Caiipa:   Automated large-scale mobile app testing through contextual fuzzing}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8576654/}{Automated   hybrid analysis of android malware through augmenting fuzzing with forced   execution}","cspan":1,"rspan":1,"markup":[1,160]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://arxiv.org/abs/2008.03585}{Automated   Functional Fuzzing of Android Apps}","cspan":1,"rspan":1,"markup":[1,87]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8708183/}{Fuzzing   the Android Applications With HTTP/HTTPS Network Data}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s10664-019-09725-6}{Evolutionary   Fuzzing of Android OS Vendor System Services}","cspan":1,"rspan":1,"markup":[1,128]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.koreascience.or.kr/article/JAKO201835372300685.page}{A   Practical Intent Fuzzing Tool for Robustness of Inter-Component Communication   in Android Apps}","cspan":1,"rspan":1,"markup":[1,171]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://paper.seebug.org/papers/Security%20Conf/Blackhat/2015/us-15-Gong-Fuzzing-Android-System-Services-By-Binder-Call-To-Escalate-Privilege.pdf}{Fuzzing   android system services by binder call to escalate privilege}","cspan":1,"rspan":1,"markup":[1,224]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8371326/}{Fuzzing:   State of the art}","cspan":1,"rspan":1,"markup":[1,90]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8854702/}{Efficient   Evolutionary Fuzzing for Android Application Installation Process}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.koreascience.or.kr/article/JAKO201509057414553.page}{Method   of Fuzzing Document Application Based on Android Devices}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6228986/}{A   whitebox approach for automated security testing of Android applications on   the cloud}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590316}{IntentFuzzer:   detecting capability leaks of android applications}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity12/technical-sessions/presentation/yan}{Droidscope:   Seamlessly reconstructing the OS and dalvik semantic views for dynamic   android malware analysis}","cspan":1,"rspan":1,"markup":[1,206]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0045790617303087}{Machine   learning aided Android malware classification}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3017427}{The   evolution of android malware and android analysis techniques}","cspan":1,"rspan":1,"markup":[1,117]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=AJXaBAAAQBAJ&oi=fnd&pg=PP1&dq=android+malware+analysis&ots=JhPi5K11rN&sig=ipShxoH8rMu6GRQ6hJRY1KRZ6hg}{Android   malware and analysis}","cspan":1,"rspan":1,"markup":[1,184]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s10586-017-0944-y}{Deep   neural architectures for large scale android malware analysis}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8293854/}{Android   malware familial classification and representative sample selection via   frequent subgraph analysis}","cspan":1,"rspan":1,"markup":[1,173]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6814679/}{Droid   permission miner: Mining prominent permissions for Android malware analysis}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6298136/}{Droidmat:   Android malware detection through manifest and api calls tracing}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s11036-019-01248-0}{AdDroid:   rule-based machine learning framework for android malware analysis}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-24018-3_12}{How   current android malware seeks to evade automated code analysis}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8770262/}{Ctdroid:   leveraging a corpus of technical blogs for android malware analysis}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6128277/}{Kernel-based   behavior analysis for android malware detection}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7516385/}{Machine   learning classifiers for android malware analysis}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7272933/}{Machine   learning based hybrid behavior models for Android malware analysis}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2799979.2800003}{DRACO:   DRoid analyst combo an android malware analysis framework}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.artificialstudios.org/alessandro.reina/pubs/eurosec13.pdf}{A   system call-centric analysis and stimulation technique to automatically   reconstruct android malware behaviors}","cspan":1,"rspan":1,"markup":[1,193]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2635868.2635869}{Apposcopy:   Semantics-based detection of android malware through static analysis}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2592791.2592796}{Rage   against the virtual machine: hindering dynamic analysis of android malware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2924715.2924719}{ScanMe   mobile: a cloud-based Android malware analysis service}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-60876-1_12}{Deep   ground truth analysis of current android malware}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2046707.2046779}{Android   permissions demystified}","cspan":1,"rspan":1,"markup":[1,92]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2295136.2295141}{Android   permissions: a perspective combining risks and benefits}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2335356.2335360}{Android   permissions: User attention, comprehension, and behavior}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-642-34638-5_6}{A   conundrum of permissions: installing applications on an android smartphone}","cspan":1,"rspan":1,"markup":[1,148]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2381934.2381938}{Dr.   android and mr. hide: fine-grained permissions in android applications}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6258449/}{Analysis   of android applications' permissions}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-642-39256-6_15}{Quantitative   security risk assessment of android permissions and applications}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://arxiv.org/abs/1303.0857}{Longitudinal   analysis of android ad library permissions}","cspan":1,"rspan":1,"markup":[1,97]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity15/technical-sessions/presentation/wijesekera}{Android   permissions remystified: A field study on contextual integrity}","cspan":1,"rspan":1,"markup":[1,174]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6693128/}{Flow   permissions for android}","cspan":1,"rspan":1,"markup":[1,93]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6529497/}{Studying   the effectiveness of android application permissions requests}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/legacy/events/webapps11/tech/final_files/webapps11_proceedings.pdf#page=83}{The   effectiveness of application permissions}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6624000/}{Asking   for (and about) permissions used by android apps}","cspan":1,"rspan":1,"markup":[1,120]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-642-30244-2_4}{Android   security permissions–can we trust them?}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://spiral.imperial.ac.uk/handle/10044/1/64236}{Resolving   the predicament of android custom permissions}","cspan":1,"rspan":1,"markup":[1,116]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=DuC64OoJSGQC&oi=fnd&pg=PR3&dq=android+permissions&ots=CdApbDguTE&sig=wpdRxBAAgsK0YC1Lrb735uMh8aA}{Application   Security for the Android Platform: Processes, Permissions, and Other   Safeguards}","cspan":1,"rspan":1,"markup":[1,244]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2420950.2420956}{Permission   evolution in the android ecosystem}","cspan":1,"rspan":1,"markup":[1,106]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.igi-global.com/article/a-novel-security-framework-for-managing-android-permissions-using-blockchain-technology/196191}{A   novel security framework for managing android permissions using blockchain   technology}","cspan":1,"rspan":1,"markup":[1,229]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7009096/}{Static   detection of Android malware by using permissions and API calls}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3197231.3197236}{An   investigation into Android run-time permissions from the end users'   perspective}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6359654/}{Android   privacy}","cspan":1,"rspan":1,"markup":[1,80]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-642-30921-2_17}{AndroidLeaks:   automatically detecting potential privacy leaks in android applications on a   large scale}","cspan":1,"rspan":1,"markup":[1,177]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7194581/}{Iccta:   Detecting inter-component privacy leaks in android apps}","cspan":1,"rspan":1,"markup":[1,127]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.298.7556&rep=rep1&type=pdf}{Investigating   user privacy in android ad libraries}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.706.5640&rep=rep1&type=pdf}{ScanDal:   Static analyzer for detecting privacy leaks in android applications}","cspan":1,"rspan":1,"markup":[1,171]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2508859.2516676}{Appintent:   Analyzing sensitive data transmission in android for privacy leakage   detection}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2245276.2232009}{A   framework for static detection of privacy leaks in android applications}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-07076-6_2}{Assessing   privacy risks in android: A user-centric approach}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2435349.2435380}{Appprofiler:   a flexible method of exposing privacy-related behavior in android   applications to end users}","cspan":1,"rspan":1,"markup":[1,167]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2766498.2766506}{Securacy:   an empirical investigation of Android applications' network usage, privacy   and security}","cspan":1,"rspan":1,"markup":[1,160]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2884781.2884855}{Toward   a framework for detecting privacy policy violations in android application   code}","cspan":1,"rspan":1,"markup":[1,149]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity13/technical-sessions/presentation/bugiel}{Flexible   and fine-grained mandatory access control on android for diverse security and   privacy policies}","cspan":1,"rspan":1,"markup":[1,205]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://journals.sagepub.com/doi/abs/10.1177/1461444817702397}{Platform   privacies: Governance, collaboration, and the different meanings of “privacy”   in iOS and Android development}","cspan":1,"rspan":1,"markup":[1,191]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2468356.2468502}{Android   and iOS users' differences concerning security and privacy}","cspan":1,"rspan":1,"markup":[1,127]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2766498.2766507}{DroidJust:   Automated functionality-aware privacy leakage analysis for Android   applications}","cspan":1,"rspan":1,"markup":[1,153]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/soups2016/workshop-program/wpi/presentation/rajivan}{Influence   of privacy attitude and privacy cue framing on android app choices}","cspan":1,"rspan":1,"markup":[1,172]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2470654.2466466}{Privacy   as part of the app decision-making process}","cspan":1,"rspan":1,"markup":[1,111]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S2214212618304356}{Dynamic   privacy leakage analysis of Android third-party libraries}","cspan":1,"rspan":1,"markup":[1,143]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1404.7431}{I   know what leaked in your pocket: uncovering privacy leaks on Android Apps   with Static Taint Analysis}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://lib.dr.iastate.edu/cgi/viewcontent.cgi?article=1233&context=creativecomponents}{An   Investigative Study on Android Verified Boot Process}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=y11NBQAAQBAJ&oi=fnd&pg=PR5&dq=android+verified+boot&ots=nWTwHPvQ4G&sig=TVJBtqqHX9qpjj0KA2X1Eb0JY7g}{Android   security internals: An in-depth guide to Android's security architecture}","cspan":1,"rspan":1,"markup":[1,233]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2808117.2808126}{Android   rooting: Methods, detection, and evasion}","cspan":1,"rspan":1,"markup":[1,109]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/woot17/workshop-program/presentation/hay}{fastboot   oem vuln: Android bootloader vulnerabilities in vendor customizations}","cspan":1,"rspan":1,"markup":[1,163]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1904.05572}{The   android platform security model}","cspan":1,"rspan":1,"markup":[1,78]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://odr.chalmers.se/handle/20.500.12380/251869}{Verified   boot in embedded systems with hard boot time constraints}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0950705118301424}{A   novel pattern recognition system for detecting Android malware by analyzing   suspicious boot sequences}","cspan":1,"rspan":1,"markup":[1,183]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://denx.de/wiki/pub/U-Boot/OpenSourceIndia2013/Multi_image_booting_scenarios.pdf}{U-Boot–Multi   image booting scenarios}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3124680.3124732}{Dm-x:   protecting volume-level integrity for cloud volumes and local block devices}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-1-4842-6106-4_6}{OS   Resiliency}","cspan":1,"rspan":1,"markup":[1,85]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6743201/}{Fast   boot and fast shutdown of Android on the embedded system}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.academia.edu/download/53217693/A_Research_On_Android_Technology_With_New_Version_Naugat7.0_7.1.pdf}{A   Research On Android Technology With New Version Naugat (7.0, 7.1)}","cspan":1,"rspan":1,"markup":[1,188]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.linuxsecrets.com/elinux-wiki/images/d/d0/Android_OTA_Updates.pdf}{Android*   Software Updates}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-47063-4_2}{Controlled   Android application execution for the IoT infrastructure}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.academia.edu/download/56785475/IRJET-V5I3269.pdf}{Recent   versions on android and survey on the versions lollipop, marshmallow and   nougat}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ipv4.delaat.net/rp/2013-2014/p40/report.pdf}{Android   patching}","cspan":1,"rspan":1,"markup":[1,78]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sae.org/publications/technical-papers/content/2020-01-1365/}{Android   Defense in Depth Strategy in an Automobile Ecosystem}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3019612.3019934}{Analysing   the vulnerability exploitation in Android with the device-mapper-verity   (dm-verity) student research abstract}","cspan":1,"rspan":1,"markup":[1,182]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7962391/}{Euphony:   Harmonious unification of cacophonous anti-virus vendor labels for android   malware}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://arxiv.org/abs/1904.05572}{The   android platform security model}","cspan":1,"rspan":1,"markup":[1,78]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://search.proquest.com/openview/ec6c009a0a3f7ef3b2b895605d995aec/1?pq-origsite=gscholar&cbl=2032677}{Simulating   Electronic Circuits on Android Device using Virtual Bread Board}","cspan":1,"rspan":1,"markup":[1,189]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-981-15-9031-3_23}{An   Android Data Protection Scheme for System-as-Root Architectures}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-32022-5_15}{Automation   of the municipal inspection process in Ecuador applying mobile-D for android}","cspan":1,"rspan":1,"markup":[1,160]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.researchgate.net/profile/Nuuva_Yusuf/publication/344642318_Android_Application_Model_of_Whats_Dating_Violence_as_an_Innovation_to_Increase_the_Knowledge_among_Adolescents/links/5f86aad7a6fdccfd7b5fc918/Android-Application-Model-of-Whats-Dating-Violence-as-an-Innovation-to-Increase-the-Knowledge-among-Adolescents.pdf}{Android   Application Model of “What‟ s Dating Violence” as an Innovation to Increase   the Knowledge among Adolescents}","cspan":1,"rspan":1,"markup":[1,457]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://orbilu.uni.lu/handle/10993/39903}{Creating   better ground truth to further understand Android malware: A large scale   mining approach based on antivirus labels and malicious artifacts}","cspan":1,"rspan":1,"markup":[1,200]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=wdW1DwAAQBAJ&oi=fnd&pg=PA155&dq=android+avb&ots=6kH9nnPXJ-&sig=0kPrf-CV3XeruhZrO6J9w-gqW8E}{Automation   of the Municipal Inspection Process in Ecuador Applying Mobile-D for Android}","cspan":1,"rspan":1,"markup":[1,232]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-1-4842-6106-4_6}{OS   Resiliency}","cspan":1,"rspan":1,"markup":[1,85]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://repositorio.unb.br/handle/10482/39901}{Metodologia   para reconstrução de dados em dispositivos móveis com Sistema Operacional   Android mediante aplicação de técnicas ISP e Combination firmware}","cspan":1,"rspan":1,"markup":[1,209]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S097535831233009X}{Reverse   Wenckebach “pseudo-supernormal” conduction or paroxysmal atrioventricular   block}","cspan":1,"rspan":1,"markup":[1,167]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://riunet.upv.es/bitstream/handle/10251/11535/memoria.pdf?sequence=1}{Android   download and search service}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://www.e-journal.janabadra.ac.id/index.php/PSN/article/view/502}{Aplikasi   Gamelan Jawa Berbasis Android}","cspan":1,"rspan":1,"markup":[1,116]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://pubs.asha.org/doi/abs/10.1044/2016_AJSLP-15-0187}{Integration   of motor learning principles into real-time ambulatory voice biofeedback and   example implementation via a clinical case study with vocal fold nodules}","cspan":1,"rspan":1,"markup":[1,230]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/article/10.1134/S2079057016030085}{Association   of aging-related obesity and metabolic syndrome in men}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7066494/}{Androi-based   C&D (connected & downloadable) IVI (in-vehicle infotainment)   platform}","cspan":1,"rspan":1,"markup":[1,149]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3019612.3019934}{Analysing   the vulnerability exploitation in Android with the device-mapper-verity   (dm-verity) student research abstract}","cspan":1,"rspan":1,"markup":[1,182]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2818000.2818036}{Baredroid:   Large-scale analysis of android apps on real devices}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3124680.3124732}{Dm-x:   protecting volume-level integrity for cloud volumes and local block devices}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.linuxsecrets.com/elinux-wiki/images/d/d0/Android_OTA_Updates.pdf}{Android*   Software Updates}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-47063-4_2}{Controlled   Android application execution for the IoT infrastructure}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://homepages.staff.os3.nl/~delaat/rp/2015-2016/p30/report.pdf}{Subverting   Android 6.0 fingerprint authentication}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2994459.2994470}{Secure   containers in Android: the Samsung KNOX case study}","cspan":1,"rspan":1,"markup":[1,118]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/woot17/workshop-program/presentation/hay}{fastboot   oem vuln: Android bootloader vulnerabilities in vendor customizations}","cspan":1,"rspan":1,"markup":[1,163]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ipv4.delaat.net/rp/2013-2014/p40/report.pdf}{Android   patching}","cspan":1,"rspan":1,"markup":[1,78]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-1-4842-6106-4_6}{OS   Resiliency}","cspan":1,"rspan":1,"markup":[1,85]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sae.org/publications/technical-papers/content/2020-01-1365/}{Android   Defense in Depth Strategy in an Automobile Ecosystem}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://ictactjournals.in/paper/IJCT_Paper_1_863_to_867.pdf}{Analysis   of android vulnerabilities and modern exploitation techniques}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=y11NBQAAQBAJ&oi=fnd&pg=PR5&dq=android+%22dm+verity%22&ots=nWTwHPvR4G&sig=_-d7Cdyyir3JNN5l6Q1zQQ3LhxA}{Android   security internals: An in-depth guide to Android's security architecture}","cspan":1,"rspan":1,"markup":[1,235]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://work.delaat.net/rp/2016-2017/p45/report.pdf}{Android   7 File Based Encryption and the Attacks Against It}","cspan":1,"rspan":1,"markup":[1,120]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/linuxfastsummit18/presentation/tso}{File   System-level Integrity Protection}","cspan":1,"rspan":1,"markup":[1,117]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://trepo.tuni.fi/bitstream/handle/123456789/24231/Parviainen.pdf?sequence=3}{Android   Camera Tuning Application}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9153399/}{Hybrid   firmware analysis for known mobile and iot security vulnerabilities}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/hernandez}{BigMAC:   Fine-Grained Policy Analysis of Android Firmware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8947099/}{Detect   malware in android firmware based on distributed network environment}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8787829/}{Toward   Automated Firmware Analysis in the IoT Era}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S014036641731294X}{The   Nexmon firmware analysis and modification framework: Empowering researchers   to enhance Wi-Fi devices}","cspan":1,"rspan":1,"markup":[1,184]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity18/presentation/tian}{Attention   spanned: Comprehensive vulnerability analysis of AT commands within the   android ecosystem}","cspan":1,"rspan":1,"markup":[1,180]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/content/pdf/10.1007/s11277-016-3618-9.pdf}{Vulnerabilities   of android OS-based telematics system}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://hernan.de/u/papers/Toward_Automated_Firmware_Analysis_in_the_IoT_Era.pdf}{Toward   Automated Firmware Analysis in the IoT Era}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/ielaam/8013/8821441/8787829-aam.pdf}{Towards   Automated Firmware Analysis in the IoT Era}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=i-yWIVd4z7MC&oi=fnd&pg=PP1&dq=android+firmware+analysis&ots=L_t-6GyyOm&sig=dBwut0XRYe4TCyNZFgGJGyo8gAE}{Android   forensics: investigation, analysis and mobile security for Google Android}","cspan":1,"rspan":1,"markup":[1,238]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8823941/}{Proxray:   Protocol model learning and guided firmware analysis}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/elsabagh}{FIRMSCOPE:   Automatic Uncovering of Privilege-Escalation Vulnerabilities in Pre-Installed   Apps in Android Firmware}","cspan":1,"rspan":1,"markup":[1,198]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.mdpi.com/2079-9292/8/1/91}{Assessment   of dual frequency GNSS observations from a Xiaomi Mi 8 Android smartphone and   positioning performance analysis}","cspan":1,"rspan":1,"markup":[1,171]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.295.7508&rep=rep1&type=pdf}{Android   anti-virus analysis}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3017427}{The   evolution of android malware and android analysis techniques}","cspan":1,"rspan":1,"markup":[1,117]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590313}{DroidRay:   a security evaluation system for customized android firmwares}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7446031/}{Andrubis--1,000,000   apps later: A view on current Android malware behaviors}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0950584917302987}{Static   analysis of android apps: A systematic literature review}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2976749.2978370}{Scalable   graph-based bug search for firmware images}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/elsabagh}{FIRMSCOPE:   Automatic Uncovering of Privilege-Escalation Vulnerabilities in Pre-Installed   Apps in Android Firmware}","cspan":1,"rspan":1,"markup":[1,198]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8947099/}{Detect   malware in android firmware based on distributed network environment}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9153399/}{Hybrid   firmware analysis for known mobile and iot security vulnerabilities}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7446031/}{Andrubis--1,000,000   apps later: A view on current Android malware behaviors}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7962474/}{Sensitive   data leakage detection in pre-installed applications of custom Android   firmware}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity18/presentation/tian}{Attention   spanned: Comprehensive vulnerability analysis of AT commands within the   android ecosystem}","cspan":1,"rspan":1,"markup":[1,180]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-58469-0_16}{Towards   automated classification of firmware images and identification of embedded   devices}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-93411-2_6}{Binarm:   Scalable and efficient detection of vulnerabilities in firmware images of   intelligent electronic devices}","cspan":1,"rspan":1,"markup":[1,186]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167739X19308490}{Static   malware detection and attribution in android byte-code through an end-to-end   deep system}","cspan":1,"rspan":1,"markup":[1,175]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity14/technical-sessions/presentation/costin}{A   large-scale analysis of the security of embedded firmwares}","cspan":1,"rspan":1,"markup":[1,160]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8418369/}{The   university of sussex-huawei locomotion and transportation dataset for   multimodal analytics with mobile devices}","cspan":1,"rspan":1,"markup":[1,181]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9229869/}{Abusing   Android Runtime for Application Obfuscation}","cspan":1,"rspan":1,"markup":[1,116]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-98446-9_35}{Evaluation   of tree based machine learning classifiers for android malware detection}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6234407/}{Dissecting   android malware: Characterization and evolution}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3301326.3301390}{Evaluating   machine learning models for android malware detection: a comparison study}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8433203/}{Efficient   signature generation for classifying cross-architecture IoT malware}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3330482.3330522}{Proposing   Automatic Dataset Generation System to Support Android Sensitive Data Leakage   Detection Systems}","cspan":1,"rspan":1,"markup":[1,168]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590312}{Efficient,   context-aware privacy leakage confinement for android applications without   firmware modding}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2307636.2307663}{Riskranker:   scalable and accurate zero-day android malware detection}","cspan":1,"rspan":1,"markup":[1,129]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/clements}{HALucinator:   Firmware re-hosting through abstraction layer emulation}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6234407/}{Dissecting   android malware: Characterization and evolution}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0956566318304755}{Cost-effective   smartphone-based reconfigurable electrochemical instrument for alcohol   determination in whole blood samples}","cspan":1,"rspan":1,"markup":[1,202]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://www.csd.uoc.gr/~hy558/papers/mal_apps.pdf}{Hey,   you, get off of my market: detecting malicious apps in official and   alternative android markets.}","cspan":1,"rspan":1,"markup":[1,162]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590313}{DroidRay:   a security evaluation system for customized android firmwares}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7801876/}{Monet:   a user-oriented behavior-based malware variants detection system for android}","cspan":1,"rspan":1,"markup":[1,148]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2660267.2660359}{Semantics-aware   android malware classification using weighted contextual api dependency   graphs}","cspan":1,"rspan":1,"markup":[1,157]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3291061}{A   close look at a daily dataset of malware samples}","cspan":1,"rspan":1,"markup":[1,103]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7962474/}{Sensitive   data leakage detection in pre-installed applications of custom Android   firmware}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3301326.3301390}{Evaluating   machine learning models for android malware detection: a comparison study}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3381991.3395608}{Parallel   Space Traveling: A Security Analysis of App-Level Virtualization in Android}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2976749.2978370}{Scalable   graph-based bug search for firmware images}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-98446-9_35}{Evaluation   of tree based machine learning classifiers for android malware detection}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7446031/}{Andrubis--1,000,000   apps later: A view on current Android malware behaviors}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-15462-2_12}{Breaking   all the things—A systematic survey of firmware extraction techniques for IoT   devices}","cspan":1,"rspan":1,"markup":[1,168]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/hernandez}{BigMAC:   Fine-Grained Policy Analysis of Android Firmware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3063955.3063981}{Android   digital forensics: data, extraction and analysis}","cspan":1,"rspan":1,"markup":[1,117]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity18/presentation/tian}{Attention   spanned: Comprehensive vulnerability analysis of AT commands within the   android ecosystem}","cspan":1,"rspan":1,"markup":[1,180]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://repositum.tuwien.at/handle/20.500.12708/2673}{Human   assisted information extraction through Bluetooth low energy on android}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8931782/}{A   firmware code gene extraction technology for IoT terminal}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.mdpi.com/2076-3417/10/12/4231}{Methodology   for Forensics Data Reconstruction on Mobile Devices with Android Operating   System Applying In-System Programming and Combination Firmware}","cspan":1,"rspan":1,"markup":[1,203]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3349623.3355477}{Free   your CSI: A channel state information extraction platform for modern Wi-Fi   chipsets}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://search.proquest.com/openview/b0b2e9cb242bda4074a221dc912cfb22/1?pq-origsite=gscholar&cbl=1686341}{Automatic   feature extraction, categorization and detection of malicious code in Android   applications}","cspan":1,"rspan":1,"markup":[1,217]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.academia.edu/download/16807224/Thesis.pdf}{Android   forensic capability and evaluation of extraction tools}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://docs.lib.purdue.edu/open_access_theses/615/}{WeChat   forensic artifacts: Android phone extraction and analysis}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8787829/}{Toward   Automated Firmware Analysis in the IoT Era}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://iopscience.iop.org/article/10.1088/1757-899X/771/1/012024/meta}{Logical   Acquisition in the Forensic Investigation Process of Android Smartphones   based on Agent using Open Source Software}","cspan":1,"rspan":1,"markup":[1,205]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S014036641731294X}{The   Nexmon firmware analysis and modification framework: Empowering researchers   to enhance Wi-Fi devices}","cspan":1,"rspan":1,"markup":[1,184]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9153399/}{Hybrid   firmware analysis for known mobile and iot security vulnerabilities}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=2qo6AwAAQBAJ&oi=fnd&pg=PR25&dq=android+firmware+extraction&ots=0nuNRfi7kZ&sig=TfPFqY-AIqect_P-2ZdE5Qhrw_A}{Android   hacker's handbook}","cspan":1,"rspan":1,"markup":[1,185]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7813792/}{Android   phone forensic: Tools and techniques}","cspan":1,"rspan":1,"markup":[1,109]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.uit.edu.mm/storage/2020/09/No.-4.pdf}{ADetect:   Hybrid Analysis Feature Extraction for Android malware Detection}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://papers.ssrn.com/sol3/papers.cfm?abstract_id=3356336}{Android   Forensics: Tools and Techniques for Manual Data Extraction}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3395351.3399360}{BaseSAFE:   baseband sanitized fuzzing through emulation}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/ruge}{Frankenstein:   Advanced Wireless Fuzzing to Exploit New Bluetooth Escalation Targets}","cspan":1,"rspan":1,"markup":[1,162]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3133956.3134069}{Difuze:   Interface aware fuzzing for kernel drivers}","cspan":1,"rspan":1,"markup":[1,111]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.cspensky.info/pdfs/ndss2019_04A-1_Song_paper.pdf}{Periscope:   An effective probing and fuzzing framework for the hardware-os boundary}","cspan":1,"rspan":1,"markup":[1,153]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.ndss-symposium.org/wp-content/uploads/2020/02/24018-paper.pdf}{HFL:   Hybrid fuzzing on the linux kernel}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/hernandez}{BigMAC:   Fine-Grained Policy Analysis of Android Firmware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/song}{Agamotto:   Accelerating Kernel Driver Fuzzing with Lightweight Virtual Machine   Checkpoints}","cspan":1,"rspan":1,"markup":[1,170]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152767/}{Ex-vivo   dynamic analysis framework for Android device drivers}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://onlinelibrary.wiley.com/doi/abs/10.1002/cpe.5756}{Fw‐fuzz:   A code coverage‐guided fuzzing framework for network protocols on firmware}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8371326/}{Fuzzing:   State of the art}","cspan":1,"rspan":1,"markup":[1,90]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8368433/}{Vulnerability   detection in iot firmware: A survey}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/elsabagh}{FIRMSCOPE:   Automatic Uncovering of Privilege-Escalation Vulnerabilities in Pre-Installed   Apps in Android Firmware}","cspan":1,"rspan":1,"markup":[1,198]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/woot20/presentation/fioraldi}{AFL++:   Combining incremental steps of fuzzing research}","cspan":1,"rspan":1,"markup":[1,127]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8708183/}{Fuzzing   the Android Applications With HTTP/HTTPS Network Data}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8923779/}{Kernel   vulnerability analysis: a survey}","cspan":1,"rspan":1,"markup":[1,104]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity18/presentation/talebi}{Charm:   Facilitating dynamic analysis of device drivers of mobile systems}","cspan":1,"rspan":1,"markup":[1,153]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1742287617303948}{New   flash memory acquisition methods based on firmware update protocols for LG   Android smartphones}","cspan":1,"rspan":1,"markup":[1,178]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3319535.3363212}{Slake:   facilitating slab manipulation for exploiting vulnerabilities in the Linux   kernel}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/hernandez}{BigMAC:   Fine-Grained Policy Analysis of Android Firmware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-15462-2_12}{Breaking   all the things—A systematic survey of firmware extraction techniques for IoT   devices}","cspan":1,"rspan":1,"markup":[1,168]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://proceeding.vap.ac.vn/index.php/proceedingvap/article/view/2017.00011}{DETECT   SECURITY THREAT IN ANDROID CUSTOM FIRMWARE BY ANALYZING APPLICATIONS   FRAMEWORK AND DEFAULT SETTINGS}","cspan":1,"rspan":1,"markup":[1,194]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8947099/}{Detect   malware in android firmware based on distributed network environment}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7881801/}{Welcome   to Binder: A kernel level attack model for the Binder in Android operating   system}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1742287617301317}{Live   acquisition of main memory data from Android smartphones and smartwatches}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3063955.3063981}{Android   digital forensics: data, extraction and analysis}","cspan":1,"rspan":1,"markup":[1,117]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-46279-0_19}{A   tool for volatile memory acquisition from Android devices}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=2qo6AwAAQBAJ&oi=fnd&pg=PR25&dq=android+firmware+kernel+extraction&ots=0nuNRfi8dZ&sig=ogyMcRCJtQfOIPdNwJRZOlThU4M}{Android   hacker's handbook}","cspan":1,"rspan":1,"markup":[1,192]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8585583/}{A   Novel approach for bootkit detection in Android Platform}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity18/presentation/tian}{Attention   spanned: Comprehensive vulnerability analysis of AT commands within the   android ecosystem}","cspan":1,"rspan":1,"markup":[1,180]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590313}{DroidRay:   a security evaluation system for customized android firmwares}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3349623.3355477}{Free   your CSI: A channel state information extraction platform for modern Wi-Fi   chipsets}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://search.proquest.com/openview/ac7e946ecfb8249c1ee9695183004121/1?pq-origsite=gscholar&cbl=1976342}{Mobile   root exploit detection based on system events extracted from android   platform}","cspan":1,"rspan":1,"markup":[1,201]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ijict.itrc.ac.ir/article-1-37-en.html}{An   Attack-Defense Model for the Binder on the Android Kernel Level}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8931782/}{A   firmware code gene extraction technology for IoT terminal}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3133956.3134069}{Difuze:   Interface aware fuzzing for kernel drivers}","cspan":1,"rspan":1,"markup":[1,111]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.mdpi.com/2076-3417/10/12/4231}{Methodology   for Forensics Data Reconstruction on Mobile Devices with Android Operating   System Applying In-System Programming and Combination Firmware}","cspan":1,"rspan":1,"markup":[1,203]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/hernandez}{BigMAC:   Fine-Grained Policy Analysis of Android Firmware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/elsabagh}{FIRMSCOPE:   Automatic Uncovering of Privilege-Escalation Vulnerabilities in Pre-Installed   Apps in Android Firmware}","cspan":1,"rspan":1,"markup":[1,198]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7446031/}{Andrubis--1,000,000   apps later: A view on current Android malware behaviors}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3191737}{Anatomy   of a vulnerable fitness tracking system: Dissecting the fitbit cloud, app,   and firmware}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2307636.2307663}{Riskranker:   scalable and accurate zero-day android malware detection}","cspan":1,"rspan":1,"markup":[1,129]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-15462-2_12}{Breaking   all the things—A systematic survey of firmware extraction techniques for IoT   devices}","cspan":1,"rspan":1,"markup":[1,168]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8947099/}{Detect   malware in android firmware based on distributed network environment}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590313}{DroidRay:   a security evaluation system for customized android firmwares}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7962474/}{Sensitive   data leakage detection in pre-installed applications of custom Android   firmware}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://www.csd.uoc.gr/~hy558/papers/mal_apps.pdf}{Hey,   you, get off of my market: detecting malicious apps in official and   alternative android markets.}","cspan":1,"rspan":1,"markup":[1,162]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2133601.2133640}{Detecting   repackaged smartphone applications in third-party android marketplaces}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7849904/}{ADROIT:   Android malware detection using meta-information}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2766498.2766508}{Droideagle:   seamless detection of visually similar android apps}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3063955.3063981}{Android   digital forensics: data, extraction and analysis}","cspan":1,"rspan":1,"markup":[1,117]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2660267.2660359}{Semantics-aware   android malware classification using weighted contextual api dependency   graphs}","cspan":1,"rspan":1,"markup":[1,157]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8787829/}{Toward   Automated Firmware Analysis in the IoT Era}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0950584916300386}{Effective   detection of android malware based on the usage of data flow APIs and machine   learning}","cspan":1,"rspan":1,"markup":[1,176]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://proceeding.vap.ac.vn/index.php/proceedingvap/article/view/2017.00011}{DETECT   SECURITY THREAT IN ANDROID CUSTOM FIRMWARE BY ANALYZING APPLICATIONS   FRAMEWORK AND DEFAULT SETTINGS}","cspan":1,"rspan":1,"markup":[1,194]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/elsabagh}{FIRMSCOPE:   Automatic Uncovering of Privilege-Escalation Vulnerabilities in Pre-Installed   Apps in Android Firmware}","cspan":1,"rspan":1,"markup":[1,198]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1084804520300527}{Pleasure   or pain? An evaluation of the costs and utilities of bloatware applications   in android smartphones}","cspan":1,"rspan":1,"markup":[1,187]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7551989/}{Jred:   Program customization and bloatware mitigation based on static analysis}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2897845.2897904}{Checking   intent-based communication in android with intent space analysis}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=cfOBDwAAQBAJ&oi=fnd&pg=PP1&dq=android+%22pre+installed%22+apps+bloatware+analysis&ots=4UlpN2dpIW&sig=rCZMNtfbA9lkOQg41tI3pzdx58g}{Learning   Android Forensics: Analyze Android devices with the latest forensic tools and   techniques}","cspan":1,"rspan":1,"markup":[1,282]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-72389-1_15}{Smartphone   bloatware: an overlooked privacy problem}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://jictra.com.pk/index.php/jictra/article/view/7}{There   is no such thing as free Lunch: An Investigation of Bloatware Effects on   Smart Devices}","cspan":1,"rspan":1,"markup":[1,157]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/2010.10088}{How   Did That Get In My Phone? Unwanted App Distribution on Android Devices}","cspan":1,"rspan":1,"markup":[1,117]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8023140/}{Ghost   installer in the shadow: Security analysis of app installation on android}","cspan":1,"rspan":1,"markup":[1,144]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2815675.2815686}{Characterizing   smartphone usage patterns from millions of android users}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=bABCDwAAQBAJ&oi=fnd&pg=PA169&dq=android+%22pre+installed%22+apps+bloatware+analysis&ots=50amIOx2Z2&sig=QK_-w9wNTbpwsXXdX6W6dbt90Q8}{Privacy   Problem}","cspan":1,"rspan":1,"markup":[1,200]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6488439/}{Do   android users write about electric sheep? examining consumer reviews in   google play}","cspan":1,"rspan":1,"markup":[1,153]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2851613.2851713}{Insights   into rooted and non-rooted android mobile devices with behavior analytics}","cspan":1,"rspan":1,"markup":[1,143]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/atc15/technical-session/presentation/martins}{Selectively   taming background android apps to improve battery lifetime}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://aaltodoc.aalto.fi/handle/123456789/27914}{Intrusion   Detection System for Android: Linux kernel system calls analysis}","cspan":1,"rspan":1,"markup":[1,133]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://www.teis-workshop.org/papers/2016/TEIS_2016_6_Geng.pdf}{Bloatware   and Jailbreaking: How Consumer-Initiated Modification Interacts with Product   Pricing}","cspan":1,"rspan":1,"markup":[1,168]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://sedici.unlp.edu.ar/handle/10915/73288}{Mobile   application development approaches: a comparative analysis on the use of   storage space}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6838907/}{Rootguard:   Protecting rooted android phones}","cspan":1,"rspan":1,"markup":[1,108]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/elsabagh}{FIRMSCOPE:   Automatic Uncovering of Privilege-Escalation Vulnerabilities in Pre-Installed   Apps in Android Firmware}","cspan":1,"rspan":1,"markup":[1,198]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7107450/}{Towards   mutation analysis of android apps}","cspan":1,"rspan":1,"markup":[1,106]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2420950.2420956}{Permission   evolution in the android ecosystem}","cspan":1,"rspan":1,"markup":[1,106]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2508859.2516689}{Vetting   undesirable behaviors in android apps with permission use analysis}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.academia.edu/download/52584050/5513797455.pdf}{System   calls analysis of malwares on android}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590313}{DroidRay:   a security evaluation system for customized android firmwares}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://arxiv.org/abs/1304.4915}{Forensic   analysis of instant messenger applications on android devices}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://re.public.polimi.it/handle/11311/1047427}{Going   native: Using a large-scale analysis of android apps to create a practical   native-code sandboxing policy}","cspan":1,"rspan":1,"markup":[1,171]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2046707.2046779}{Android   permissions demystified}","cspan":1,"rspan":1,"markup":[1,92]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2818000.2818036}{Baredroid:   Large-scale analysis of android apps on real devices}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.packetstormsecurity.net/papers/general/NDSS12_WOODPECKER.pdf}{Systematic   detection of capability leaks in stock android smartphones.}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity16/technical-sessions/presentation/aafer}{Harvesting   inconsistent security configurations in custom android roms via differential   analysis}","cspan":1,"rspan":1,"markup":[1,197]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3143361.3143400}{Studying   TLS usage in Android apps}","cspan":1,"rspan":1,"markup":[1,95]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.researchgate.net/profile/Franklin_Tchakounte/publication/271199472_Permission-based_Malware_Detection_Mechanisms_on_Android_Analysis_and_Perspectives/links/54c11b5c0cf2d03405c4de97.pdf}{Permission-based   malware detection mechanisms on android: Analysis and perspectives}","cspan":1,"rspan":1,"markup":[1,290]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.researchgate.net/profile/Hans_Hoefken/publication/260320851_Forensic_Analysis_of_Geodata_in_Android_Smartphones/links/0046353148e8fccc09000000/Forensic-Analysis-of-Geodata-in-Android-Smartphones.pdf}{Forensic   analysis of geodata in android smartphones}","cspan":1,"rspan":1,"markup":[1,272]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S174228761500002X}{APK   Auditor: Permission-based Android malware detection system}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0950584916300684}{Mutation   operators for testing Android apps}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2494603.2480308}{Insights   into layout patterns of mobile user interfaces by an automatic analysis of   android apps}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590325}{Evading   android runtime analysis via sandbox detection}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2746266.2746271}{Android   malware static analysis techniques}","cspan":1,"rspan":1,"markup":[1,103]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://re.public.polimi.it/handle/11311/1047427}{Going   native: Using a large-scale analysis of android apps to create a practical   native-code sandboxing policy}","cspan":1,"rspan":1,"markup":[1,171]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/elsabagh}{FIRMSCOPE:   Automatic Uncovering of Privilege-Escalation Vulnerabilities in Pre-Installed   Apps in Android Firmware}","cspan":1,"rspan":1,"markup":[1,198]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590313}{DroidRay:   a security evaluation system for customized android firmwares}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2420950.2420956}{Permission   evolution in the android ecosystem}","cspan":1,"rspan":1,"markup":[1,106]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2046707.2046779}{Android   permissions demystified}","cspan":1,"rspan":1,"markup":[1,92]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7557676/}{Merging   permission and api features for android malware detection}","cspan":1,"rspan":1,"markup":[1,130]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7961980/}{Open   doors for bob and mallory: Open port usage in android apps and security   implications}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/1999995.2000018}{Analyzing   inter-application communication in Android}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.academia.edu/download/52584050/5513797455.pdf}{System   calls analysis of malwares on android}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2508859.2516689}{Vetting   undesirable behaviors in android apps with permission use analysis}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6280226/}{A   case study in open source software security and privacy: Android adware}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-34175-6_15}{Android   multitasking mechanism: Formal semantics and static analysis of apps}","cspan":1,"rspan":1,"markup":[1,149]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3243734.3243843}{Invetter:   Locating insecure input validations in android services}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7107450/}{Towards   mutation analysis of android apps}","cspan":1,"rspan":1,"markup":[1,106]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3143361.3143400}{Studying   TLS usage in Android apps}","cspan":1,"rspan":1,"markup":[1,95]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.packetstormsecurity.net/papers/general/NDSS12_WOODPECKER.pdf}{Systematic   detection of capability leaks in stock android smartphones.}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6531746/}{A   new android malware detection approach using bayesian classification}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.academia.edu/download/52584050/5513797455.pdf}{System   calls analysis of malwares on android}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590313}{DroidRay:   a security evaluation system for customized android firmwares}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.researchgate.net/profile/Victor_Van_Der_Veen/publication/270576401_Dynamic_Analysis_of_Android_Malware/links/54ae68470cf2828b29fcf321/Dynamic-Analysis-of-Android-Malware.pdf}{Dynamic   analysis of android malware}","cspan":1,"rspan":1,"markup":[1,231]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2897073.2897716}{Droidmate:   a robust and extensible test generator for android}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590325}{Evading   android runtime analysis via sandbox detection}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2508859.2516689}{Vetting   undesirable behaviors in android apps with permission use analysis}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/elsabagh}{FIRMSCOPE:   Automatic Uncovering of Privilege-Escalation Vulnerabilities in Pre-Installed   Apps in Android Firmware}","cspan":1,"rspan":1,"markup":[1,198]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8255546/}{Samadroid:   a novel 3-level hybrid malware detection model for android operating system}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://rasthofer.info/publications/paper/NDSS2014-SuSi.pdf}{A   machine-learning approach for classifying and categorizing android sources   and sinks.}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://re.public.polimi.it/handle/11311/1047427}{Going   native: Using a large-scale analysis of android apps to create a practical   native-code sandboxing policy}","cspan":1,"rspan":1,"markup":[1,171]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/1999995.2000018}{Analyzing   inter-application communication in Android}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6876208/}{Permission   use analysis for vetting undesirable behaviors in android apps}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2046707.2046779}{Android   permissions demystified}","cspan":1,"rspan":1,"markup":[1,92]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8038362/}{Analyzing   android application in real-time at kernel level}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2818000.2818036}{Baredroid:   Large-scale analysis of android apps on real devices}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://cs.gmu.edu/media/techreports/GMU-CS-TR-2015-5.pdf}{Automated   dynamic enforcement of synthesized security policies in android}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-13257-0_20}{Analyzing   android browser apps for file://vulnerabilities}","cspan":1,"rspan":1,"markup":[1,130]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6956578/}{The   peril of fragmentation: Security hazards in android device driver   customizations}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590313}{DroidRay:   a security evaluation system for customized android firmwares}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7557676/}{Merging   permission and api features for android malware detection}","cspan":1,"rspan":1,"markup":[1,130]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-04283-1_6}{Droidapiminer:   Mining api-level features for robust malware detection in android}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167404817300640}{PIndroid:   A novel Android malware detection system using ensemble learning methods}","cspan":1,"rspan":1,"markup":[1,160]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2420950.2420956}{Permission   evolution in the android ecosystem}","cspan":1,"rspan":1,"markup":[1,106]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.researchgate.net/profile/Franklin_Tchakounte/publication/271199472_Permission-based_Malware_Detection_Mechanisms_on_Android_Analysis_and_Perspectives/links/54c11b5c0cf2d03405c4de97.pdf}{Permission-based   malware detection mechanisms on android: Analysis and perspectives}","cspan":1,"rspan":1,"markup":[1,290]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6531746/}{A   new android malware detection approach using bayesian classification}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S174228761500002X}{APK   Auditor: Permission-based Android malware detection system}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2746266.2746271}{Android   malware static analysis techniques}","cspan":1,"rspan":1,"markup":[1,103]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6313688/}{Malicious   android applications in the enterprise: What do they do and how do we fix   it?}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6550526/}{Android   SMS malware: Vulnerability and mitigation}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1904.00736}{Using   deep neural network for Android malware detection}","cspan":1,"rspan":1,"markup":[1,98]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://www.llonely.com/goto/https://public.gdatasoftware.com/Presse/Publikationen/Malware_Reports/G_DATA_MobileMWR_Q2_2015_EN.pdf}{Mobile   malware report}","cspan":1,"rspan":1,"markup":[1,161]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7389671/}{A   study of android malware detection technology evolution}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6956577/}{Upgrading   your android, elevating my malware: Privilege escalation through mobile os   updating}","cspan":1,"rspan":1,"markup":[1,160]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.academia.edu/download/52584050/5513797455.pdf}{System   calls analysis of malwares on android}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://www.itiis.org/digital-library/manuscript/file/20858/TIISVol9No8-12.pdf}{Intelligent   Approach for Android Malware Detection.}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.researchgate.net/profile/Victor_Van_Der_Veen/publication/270576401_Dynamic_Analysis_of_Android_Malware/links/54ae68470cf2828b29fcf321/Dynamic-Analysis-of-Android-Malware.pdf}{Dynamic   analysis of android malware}","cspan":1,"rspan":1,"markup":[1,231]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7985674/}{Libd:   Scalable and precise third-party library detection in android markets}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2976749.2978333}{Reliable   third-party library detection in android and its security applications}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2889160.2889178}{Libradar:   Fast and accurate detection of third-party libraries in android apps}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6827639/}{Addetect:   Automated detection of android ad libraries using semantic analysis}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8543426/}{Orlis:   Obfuscation-resilient library detection for Android}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167404818311301}{Securing   android applications via edge assistant third-party library detection}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8330204/}{Detecting   third-party libraries in android applications with high precision and recall}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8478000/}{Large-scale   third-party library detection in android markets}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9286020/}{Automated   Third-Party Library Detection for Android Applications: Are We There Yet?}","cspan":1,"rspan":1,"markup":[1,148]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6985631/}{Andarwin:   Scalable detection of android application clones based on semantics}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3293882.3330563}{Libid:   reliable identification of obfuscated third-party android libraries}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s11277-018-5456-4}{Identify   and inspect libraries in android applications}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6665098/}{Automatic   detection of inter-application permission leaks in android applications}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/enigma2018/presentation/derr}{The   impact of third-party code on android app security}","cspan":1,"rspan":1,"markup":[1,127]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0164121219301001}{Revisiting   the impact of common libraries for android-related investigations}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7972730/}{Who   changed you? Obfuscator identification for Android}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-642-40203-6_11}{Andarwin:   Scalable detection of semantically similar android applications}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3133956.3134059}{Keep   me updated: An empirical study of third-party library updatability on   android}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2771783.2771800}{Dynamic   detection of inter-application communication vulnerabilities in Android}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6566868/}{Networkprofiler:   Towards automatic fingerprinting of android apps}","cspan":1,"rspan":1,"markup":[1,130]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s11704-017-6493-y}{Fingerprinting   Android malware families}","cspan":1,"rspan":1,"markup":[1,109]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167404820301437}{Scalable   and robust unsupervised android malware fingerprinting using community-based   network partitioning}","cspan":1,"rspan":1,"markup":[1,186]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2513228.2513331}{Design   of a mobile inspector for detecting illegal Android applications using   fingerprinting}","cspan":1,"rspan":1,"markup":[1,155]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-98989-1_4}{Investigating   Fingerprinters and Fingerprinting-Alike Behaviour of Android Applications}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://spectrum.library.concordia.ca/986733/}{Resilient   and Scalable Android Malware Fingerprinting and Detection}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://rua.ua.es/dspace/handle/10045/76082}{Android   library for recognition of activities of daily living: implementation   considerations, challenges, and solutions}","cspan":1,"rspan":1,"markup":[1,174]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8399710/}{WiFi   RSSI preprocessing library for Android}","cspan":1,"rspan":1,"markup":[1,108]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8835276/}{Sensorid:   Sensor calibration fingerprinting for smartphones}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.mdpi.com/1424-8220/21/2/432}{Development   of a Smartphone-Based University Library Navigation and Information Service   Employing Wi-Fi Location Fingerprinting}","cspan":1,"rspan":1,"markup":[1,179]},{"value":"2021","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8543426/}{Orlis:   Obfuscation-resilient library detection for Android}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8456014/}{Website   Fingerprinting by Power Estimation Based Side-Channel Attacks on Android 7}","cspan":1,"rspan":1,"markup":[1,147]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://arxiv.org/abs/1408.1416}{Mobile   device identification via sensor fingerprinting}","cspan":1,"rspan":1,"markup":[1,96]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-58469-0_23}{Binsign:   fingerprinting binary functions to support automated analysis of code   executables}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://modul.repo.mercubuana-yogya.ac.id/modul/files/openjournal/OpenJournnalOfIndustry/canvas.pdf}{Pixel   perfect: Fingerprinting canvas in HTML5}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8057232/}{POWERFUL:   Mobile app fingerprinting via power analysis}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity18/presentation/bonett}{Discovering   flaws in security-focused static analysis tools for android using systematic   mutation}","cspan":1,"rspan":1,"markup":[1,180]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7467346/}{HornDroid:   Practical and sound static analysis of Android applications by SMT solving}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2996358}{droid:   Assessment and evaluation of android application analysis tools}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7180133/}{A   dataset of open-source android applications}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0950584912001012}{Static   analysis of Android programs}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6149548/}{Android:   Static analysis using similarity distance}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3243734.3243835}{Jn-saf:   Precise and efficient ndk/jni-aware inter-language static analysis framework   for security vetting of android applications with native code}","cspan":1,"rspan":1,"markup":[1,209]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7582763/}{HybriDroid:   static analysis framework for Android hybrid applications}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3236024.3236029}{Do   android taint analysis tools keep their promises?}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8817113/}{Where   are we looking? Understanding android static analysis techniques}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2259051.2259056}{Dexpler:   converting android dalvik bytecode to jimple for static analysis with soot}","cspan":1,"rspan":1,"markup":[1,144]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0950584917302987}{Static   analysis of android apps: A systematic literature review}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3293882.3339001}{Androlic:   an extensible flow, context, object, field, and path-sensitive static   analysis framework for Android}","cspan":1,"rspan":1,"markup":[1,173]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2970276.2970277}{Reflection-aware   static analysis of android apps}","cspan":1,"rspan":1,"markup":[1,109]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8445034/}{Software   quality through the eyes of the end-user and static analysis tools: A study   on android oss applications}","cspan":1,"rspan":1,"markup":[1,179]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7446031/}{Andrubis--1,000,000   apps later: A view on current Android malware behaviors}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8539081/}{RedDroid:   Android application redundancy customization based on static analysis}","cspan":1,"rspan":1,"markup":[1,144]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8229907/}{An   app based on static analysis for Android ransomware}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8094430/}{Evaluating   state-of-the-art free and open source static analysis tools against buffer   errors in android apps}","cspan":1,"rspan":1,"markup":[1,175]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2837614.2837661}{Combining   static analysis with probabilistic models to enable market-scale android   inter-component analysis}","cspan":1,"rspan":1,"markup":[1,170]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6149548/}{Android:   Static analysis using similarity distance}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6112328/}{Using   static analysis for automatic assessment and mitigation of unwanted and   malicious activities within Android applications}","cspan":1,"rspan":1,"markup":[1,193]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7019227/}{Detecting   software vulnerabilities in android using static analysis}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0950584917302987}{Static   analysis of android apps: A systematic literature review}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://isyou.info/jisis/vol6/no4/jisis-2016-vol6-no4-03.pdf}{Android   Application Protection against Static Reverse Engineering based on   Multidexing.}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://onlinelibrary.wiley.com/doi/abs/10.1002/spe.2643}{VAnDroid:   A framework for vulnerability analysis of Android applications using a   model‐driven reverse engineering technique}","cspan":1,"rspan":1,"markup":[1,192]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2751323.2751330}{Exploring   reverse engineering symptoms in Android apps}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1631/FITEE.1601491}{Discovering   optimal features using static analysis and a genetic search based method for   Android malware detection}","cspan":1,"rspan":1,"markup":[1,182]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.mdpi.com/558048}{AndroShield:   automated android applications vulnerability detection, a hybrid static and   dynamic analysis approach}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.itc.ktu.lt/index.php/ITC/article/view/21457}{What   static analysis can utmost offer for Android malware detection}","cspan":1,"rspan":1,"markup":[1,133]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8539081/}{RedDroid:   Android application redundancy customization based on static analysis}","cspan":1,"rspan":1,"markup":[1,144]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.researchgate.net/profile/Mark-Stamp/publication/314521542_Static_and_Dynamic_Analysis_of_Android_Malware/links/5bdee8ad299bf1124fb9cab6/Static-and-Dynamic-Analysis-of-Android-Malware.pdf}{Static   and dynamic analysis of android malware.}","cspan":1,"rspan":1,"markup":[1,256]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1410.7751}{Andlantis:   Large-scale Android dynamic analysis}","cspan":1,"rspan":1,"markup":[1,89]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s10515-018-0237-6}{Static   window transition graphs for Android}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-58793-2_30}{Reverse   Engineering of Android Applications: REiMPAcT}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2259051.2259056}{Dexpler:   converting android dalvik bytecode to jimple for static analysis with soot}","cspan":1,"rspan":1,"markup":[1,144]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8716380/}{Android   applications scanning: The guide}","cspan":1,"rspan":1,"markup":[1,105]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://journal.utem.edu.my/index.php/jtec/article/view/2870}{A   hybrid approach for reverse engineering GUI model from android apps for   automated testing}","cspan":1,"rspan":1,"markup":[1,164]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6079840/}{An   Android security case study with bauhaus}","cspan":1,"rspan":1,"markup":[1,108]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-68690-5_12}{Detecting   energy bugs in android apps using static analysis}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6813664/}{Static   analysis for extracting permission checks of a large scale framework: The   challenges and solutions for analyzing android}","cspan":1,"rspan":1,"markup":[1,194]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2382196.2382222}{Pscout:   analyzing the android permission specification}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6814679/}{Droid   permission miner: Mining prominent permissions for Android malware analysis}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.researchgate.net/profile/Mark-Stamp/publication/314521542_Static_and_Dynamic_Analysis_of_Android_Malware/links/5bdee8ad299bf1124fb9cab6/Static-and-Dynamic-Analysis-of-Android-Malware.pdf}{Static   and dynamic analysis of android malware.}","cspan":1,"rspan":1,"markup":[1,256]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6494934/}{Automatically   securing permission-based software by reducing the attack surface: An   application to android}","cspan":1,"rspan":1,"markup":[1,173]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7417621/}{Reevaluating   android permission gaps with static and dynamic analysis}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2791405.2791558}{Two   phase static analysis technique for android malware detection}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7792435/}{ANASTASIA:   ANdroid mAlware detection using STatic analySIs of Applications}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2484313.2484359}{DroidAlarm:   an all-sided static analysis tool for Android privilege-escalation malware}","cspan":1,"rspan":1,"markup":[1,147]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0925231217312870}{DroidDet:   effective and robust detection of android malware using static analysis along   with rotation forest model}","cspan":1,"rspan":1,"markup":[1,194]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6735264/}{Machine   learning for android malware detection using permission and api calls}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0164121220300169}{An   Android application risk evaluation framework based on minimum permission set   identification}","cspan":1,"rspan":1,"markup":[1,175]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7203053/}{Analysis   of android inter-app security vulnerabilities using covert}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://scholarworks.sjsu.edu/etd_projects/488/}{Static   and dynamic analysis for android malware detection}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7009096/}{Static   detection of Android malware by using permissions and API calls}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-981-10-7200-0_13}{Static   and dynamic analysis for android malware detection}","cspan":1,"rspan":1,"markup":[1,130]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s12652-020-01957-5}{A   novel permission ranking system for android malware detection—the permission   grader}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://aip.scitation.org/doi/abs/10.1063/1.4992953}{An   Android malware detection system based on machine learning}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://digital-library.theiet.org/content/journals/10.1049/iet-ifs.2014.0099}{High   accuracy android malware detection using ensemble learning}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7537161/}{Detection   of android malware by static analysis on permissions and sensitive functions}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-94-007-2792-2_50}{A   study on static analysis model of mobile application for privacy protection}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://iopscience.iop.org/article/10.1088/1742-6596/1288/1/012053/meta}{Vulnerability   Parser: A Static Vulnerability Analysis System for Android Applications}","cspan":1,"rspan":1,"markup":[1,167]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6298136/}{Droidmat:   Android malware detection through manifest and api calls tracing}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2185448.2185466}{Droidchecker:   analyzing android applications for capability leak}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8697714/}{S3ntinel:   An Extensible Static Analysis Framework for Android Applications}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2837614.2837661}{Combining   static analysis with probabilistic models to enable market-scale android   inter-component analysis}","cspan":1,"rspan":1,"markup":[1,170]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2480362.2480701}{Mobile-sandbox:   having a deeper look into android applications}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3243734.3243835}{Jn-saf:   Precise and efficient ndk/jni-aware inter-language static analysis framework   for security vetting of android applications with native code}","cspan":1,"rspan":1,"markup":[1,209]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7307791/}{Android   malware detection based on static analysis of characteristic tree}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2897845.2897927}{R-droid:   Leveraging android app analysis with static slice optimization}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9283770/}{ASAF:   Android Static Analysis Framework}","cspan":1,"rspan":1,"markup":[1,104]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2484313.2484359}{DroidAlarm:   an all-sided static analysis tool for Android privilege-escalation malware}","cspan":1,"rspan":1,"markup":[1,147]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity13/technical-sessions/presentation/octeau}{Effective   inter-component communication mapping in android: An essential step towards   holistic security analysis}","cspan":1,"rspan":1,"markup":[1,214]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://people.csail.mit.edu/rinard/paper/ndss15.droidsafe.pdf}{Information   flow analysis of android applications in droidsafe.}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7446031/}{Andrubis--1,000,000   apps later: A view on current Android malware behaviors}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2382196.2382222}{Pscout:   analyzing the android permission specification}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2666356.2594299}{Flowdroid:   Precise context, flow, field, object-sensitive and lifecycle-aware taint   analysis for android apps}","cspan":1,"rspan":1,"markup":[1,172]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://digital-library.theiet.org/content/journals/10.1049/iet-ifs.2013.0095}{Analysis   of Bayesian classification-based approaches for Android malware detection}","cspan":1,"rspan":1,"markup":[1,170]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7163067/}{Effective   real-time android application auditing}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/hernandez}{BigMAC:   Fine-Grained Policy Analysis of Android Firmware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590312}{Efficient,   context-aware privacy leakage confinement for android applications without   firmware modding}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.researchgate.net/profile/Victor_Van_Der_Veen/publication/270576401_Dynamic_Analysis_of_Android_Malware/links/54ae68470cf2828b29fcf321/Dynamic-Analysis-of-Android-Malware.pdf}{Dynamic   analysis of android malware}","cspan":1,"rspan":1,"markup":[1,231]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/harrison}{PARTEMU:   Enabling Dynamic Analysis of Real-World TrustZone Software Using Emulation}","cspan":1,"rspan":1,"markup":[1,166]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3359789.3359833}{Opening   Pandora's box through ATFuzzer: dynamic analysis of AT interface for Android   smartphones}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7226692/}{Code   coverage measurement for Android dynamic analysis tools}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/elsabagh}{FIRMSCOPE:   Automatic Uncovering of Privilege-Escalation Vulnerabilities in Pre-Installed   Apps in Android Firmware}","cspan":1,"rspan":1,"markup":[1,198]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590313}{DroidRay:   a security evaluation system for customized android firmwares}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity18/presentation/talebi}{Charm:   Facilitating dynamic analysis of device drivers of mobile systems}","cspan":1,"rspan":1,"markup":[1,153]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1742287617303948}{New   flash memory acquisition methods based on firmware update protocols for LG   Android smartphones}","cspan":1,"rspan":1,"markup":[1,178]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9153399/}{Hybrid   firmware analysis for known mobile and iot security vulnerabilities}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.researchgate.net/profile/Jonas_Zaddach/publication/269197057_Avatar_A_Framework_to_Support_Dynamic_Security_Analysis_of_Embedded_Systems'_Firmwares/links/5e0b2725299bf10bc3852355/Avatar-A-Framework-to-Support-Dynamic-Security-Analysis-of-Embedded-Systems-Firmwares.pdf}{AVATAR:   A Framework to Support Dynamic Security Analysis of Embedded Systems'   Firmwares.}","cspan":1,"rspan":1,"markup":[1,381]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/clements}{HALucinator:   Firmware re-hosting through abstraction layer emulation}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8368433/}{Vulnerability   detection in iot firmware: A survey}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2939918.2939926}{Evading   android runtime analysis through detecting programmed interactions}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7446031/}{Andrubis   1,000,000 apps later: A view on current Android malware behaviors}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8787829/}{Toward   Automated Firmware Analysis in the IoT Era}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://content.iospress.com/articles/journal-of-intelligent-and-fuzzy-systems/ifs169424}{Detecting   Android malware using long short-term memory (LSTM)}","cspan":1,"rspan":1,"markup":[1,160]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8278529/}{A   collaborative framework for android malware detection using DNS & dynamic   analysis}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152633/}{An   analysis of pre-installed android software}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590313}{DroidRay:   a security evaluation system for customized android firmwares}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.academia.edu/download/52584050/5513797455.pdf}{System   calls analysis of malwares on android}","cspan":1,"rspan":1,"markup":[1,112]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.researchgate.net/profile/Victor_Van_Der_Veen/publication/270576401_Dynamic_Analysis_of_Android_Malware/links/54ae68470cf2828b29fcf321/Dynamic-Analysis-of-Android-Malware.pdf}{Dynamic   analysis of android malware}","cspan":1,"rspan":1,"markup":[1,231]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2897073.2897716}{Droidmate:   a robust and extensible test generator for android}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8255546/}{Samadroid:   a novel 3-level hybrid malware detection model for android operating system}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity20/presentation/elsabagh}{FIRMSCOPE:   Automatic Uncovering of Privilege-Escalation Vulnerabilities in Pre-Installed   Apps in Android Firmware}","cspan":1,"rspan":1,"markup":[1,198]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://rasthofer.info/publications/paper/NDSS2014-SuSi.pdf}{A   machine-learning approach for classifying and categorizing android sources   and sinks.}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2508859.2516689}{Vetting   undesirable behaviors in android apps with permission use analysis}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3278532.3278558}{Beyond   google play: A large-scale comparative study of chinese android app markets}","cspan":1,"rspan":1,"markup":[1,143]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://cs.gmu.edu/media/techreports/GMU-CS-TR-2015-5.pdf}{Automated   dynamic enforcement of synthesized security policies in android}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6956578/}{The   peril of fragmentation: Security hazards in android device driver   customizations}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://re.public.polimi.it/handle/11311/1047427}{Going   native: Using a large-scale analysis of android apps to create a practical   native-code sandboxing policy}","cspan":1,"rspan":1,"markup":[1,171]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-04283-1_6}{Droidapiminer:   Mining api-level features for robust malware detection in android}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2590296.2590325}{Evading   android runtime analysis via sandbox detection}","cspan":1,"rspan":1,"markup":[1,115]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-13257-0_20}{Analyzing   android browser apps for file://vulnerabilities}","cspan":1,"rspan":1,"markup":[1,130]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6280226/}{A   case study in open source software security and privacy: Android adware}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3300061.3345452}{Device   administrator use and abuse in Android: Detection and characterization}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.packetstormsecurity.net/papers/general/NDSS12_WOODPECKER.pdf}{Systematic   detection of capability leaks in stock android smartphones.}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2664243.2664245}{Design   and implementation of an android host-based intrusion prevention system}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6982893/}{Malware   detection using network traffic analysis in android based mobile devices}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1410.7751}{Andlantis:   Large-scale Android dynamic analysis}","cspan":1,"rspan":1,"markup":[1,89]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2940343.2940348}{CREDROID:   Android malware detection by network traffic analysis}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6657309/}{Ananas-a   framework for analyzing android applications}","cspan":1,"rspan":1,"markup":[1,118]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2480362.2480701}{Mobile-sandbox:   having a deeper look into android applications}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-72550-5_46}{Android   malware detection based on network traffic using decision tree algorithm}","cspan":1,"rspan":1,"markup":[1,153]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S016412122030087X}{Identifying   vulnerabilities of SSL/TLS certificate verification in Android apps with   static and dynamic analysis}","cspan":1,"rspan":1,"markup":[1,192]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9153400/}{LIBSPECTOR:   Context-Aware Large-Scale Network Traffic Analysis of Android Applications}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7013120/}{Comparative   study of k-means and mini batch k-means clustering algorithms in android   malware detection using network traffic analysis}","cspan":1,"rspan":1,"markup":[1,200]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2592791.2592796}{Rage   against the virtual machine: hindering dynamic analysis of android malware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7043530/}{Malware   detection in Android by network traffic analysis}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7035780/}{Manilyzer:   automated android malware detection through manifest analysis}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.mdpi.com/558048}{AndroShield:   automated android applications vulnerability detection, a hybrid static and   dynamic analysis approach}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S2214212619303837}{Visualizing   the outcome of dynamic analysis of Android malware with VizMal}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.ndss-symposium.org/wp-content/uploads/2017/09/intellidroid-targeted-input-generator-dynamic-analysis-android-malware.pdf}{IntelliDroid:   A Targeted Input Generator for the Dynamic Analysis of Android Malware.}","cspan":1,"rspan":1,"markup":[1,228]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8455983/}{NTPDroid:   a hybrid android malware detector using network traffic and system   permissions}","cspan":1,"rspan":1,"markup":[1,155]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.researchgate.net/profile/Mark-Stamp/publication/314521542_Static_and_Dynamic_Analysis_of_Android_Malware/links/5bdee8ad299bf1124fb9cab6/Static-and-Dynamic-Analysis-of-Android-Malware.pdf}{Static   and dynamic analysis of android malware.}","cspan":1,"rspan":1,"markup":[1,256]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1742287617303183}{An   in-depth analysis of Android malware using hybrid techniques}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8374030/}{A   novel dynamic Android malware detection system with ensemble learning}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s10207-014-0250-0}{Mobile-Sandbox:   combining static and dynamic analysis with machine-learning techniques}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://search.proquest.com/openview/7dedd0447f7a9400cb60eba599536da6/1?pq-origsite=gscholar&cbl=18750&diss=y}{DroidDocker:   Dynamic analysis of android applications on Docker}","cspan":1,"rspan":1,"markup":[1,183]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.worldscientific.com/doi/abs/10.1142/9789813273238_0066}{A   new tool for static and dynamic Android malware analysis}","cspan":1,"rspan":1,"markup":[1,135]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://128.171.57.22/handle/10125/64555}{Detecting   repackaged android applications using perceptual hashing}","cspan":1,"rspan":1,"markup":[1,116]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7214136/}{Dynalize:   Dynamic analysis of mobile apps in a platform-as-a-service cloud}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1877050916302873}{Scredent:   Scalable real-time anomalies detection and notification of targeted malware   in mobile devices}","cspan":1,"rspan":1,"markup":[1,183]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1566253518306778}{Android   malware detection through hybrid features fusion and ensemble classifiers:   The AndroPyTool framework and the OmniDroid dataset}","cspan":1,"rspan":1,"markup":[1,214]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8622324/}{R2-d2:   Color-inspired convolutional neural network (cnn)-based android malware   detections}","cspan":1,"rspan":1,"markup":[1,156]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://content.iospress.com/articles/journal-of-intelligent-and-fuzzy-systems/ifs169953}{Grefenstette   Bias based genetic algorithm for multi-site offloading using docker container   in edge computing}","cspan":1,"rspan":1,"markup":[1,209]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8679493/}{Analysis   and detection of malware in Android applications using machine learning}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://www.iaeng.org/IJCS/issues_v45/issue_4/IJCS_45_4_03.pdf}{Android   malware classification based on mobile security framework}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-58951-6_13}{Understanding   the Security Risks of Docker Hub}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9284058/}{Time-travel   testing of Android apps}","cspan":1,"rspan":1,"markup":[1,100]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://arxiv.org/abs/2005.10762}{Concurrency-related   flaky test detection in android apps}","cspan":1,"rspan":1,"markup":[1,99]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3329786}{Dynamic   malware analysis in the modern era. A state of the art survey}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8667832/}{An   empirical case study on the temporary file smell in dockerfiles}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8026871/}{Performance   tuning and modeling for big data applications in docker containers}","cspan":1,"rspan":1,"markup":[1,143]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://scholar.sun.ac.za/handle/10019.1/102802}{Verifying   Android Applications Using Java PathFinder}","cspan":1,"rspan":1,"markup":[1,109]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8890109/}{FastBuild:   Accelerating Docker image building for efficient development and deployment   of container}","cspan":1,"rspan":1,"markup":[1,166]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://arxiv.org/abs/1410.7751}{Andlantis:   Large-scale Android dynamic analysis}","cspan":1,"rspan":1,"markup":[1,89]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3041008.3041010}{Emulator   vs real phone: Android malware detection using machine learning}","cspan":1,"rspan":1,"markup":[1,133]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2592791.2592796}{Rage   against the virtual machine: hindering dynamic analysis of android malware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2799979.2800004}{A   robust dynamic analysis system preventing SandBox detection by Android   malware}","cspan":1,"rspan":1,"markup":[1,143]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6657309/}{Ananas-a   framework for analyzing android applications}","cspan":1,"rspan":1,"markup":[1,118]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.mdpi.com/558048}{AndroShield:   automated android applications vulnerability detection, a hybrid static and   dynamic analysis approach}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://cecs.wright.edu/~pmateti/Courses/4440/Lectures/Detection/summercon12-bouncer.pdf}{Dissecting   the android bouncer}","cspan":1,"rspan":1,"markup":[1,129]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.researchgate.net/profile/Mark-Stamp/publication/314521542_Static_and_Dynamic_Analysis_of_Android_Malware/links/5bdee8ad299bf1124fb9cab6/Static-and-Dynamic-Analysis-of-Android-Malware.pdf}{Static   and dynamic analysis of android malware.}","cspan":1,"rspan":1,"markup":[1,256]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7502337/}{DynaLog:   An automated dynamic analysis framework for characterizing android   applications}","cspan":1,"rspan":1,"markup":[1,155]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{http://ceur-ws.org/Vol-1575/paper_10.pdf}{ARTDroid:   A Virtual-Method Hooking Framework on Android ART Runtime.}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9152767/}{Ex-vivo   dynamic analysis framework for Android device drivers}","cspan":1,"rspan":1,"markup":[1,126]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7098023/}{Condroid:   Targeted dynamic analysis of android applications}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2480362.2480701}{Mobile-sandbox:   having a deeper look into android applications}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1609.04718}{Glassbox:   dynamic analysis platform for malware android applications on real devices}","cspan":1,"rspan":1,"markup":[1,127]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8326293/}{DDefender:   Android application threat detection using static and dynamic analysis}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6906344/}{DroidTrace:   A ptrace based Android dynamic analysis system with forward execution   capability}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3134600.3134601}{Droid-AntiRM:   Taming control flow anti-analysis to support automated dynamic analysis of   android malware}","cspan":1,"rspan":1,"markup":[1,167]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=72nnDwAAQBAJ&oi=fnd&pg=PA73&dq=android+dynamic+analysis+emulator&ots=42pKkKSpv8&sig=Xl8zujvsUB4AXehU6G48hDZ5DfM}{Effectiveness   of state-of-the-art dynamic analysis techniques in identifying diverse   Android malware and future enhancements}","cspan":1,"rspan":1,"markup":[1,292]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-61638-0_26}{DaVinci:   Android App Analysis Beyond Frida via Dynamic System Call Instrumentation}","cspan":1,"rspan":1,"markup":[1,155]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://ceur-ws.org/Vol-1575/paper_10.pdf}{ARTDroid:   A Virtual-Method Hooking Framework on Android ART Runtime.}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3400286.3418266}{EDAroid:   An Efficient Dynamic Analysis Tool for Android Applications}","cspan":1,"rspan":1,"markup":[1,129]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8029446/}{T2Droid:   A TrustZone-based dynamic analyser for Android applications}","cspan":1,"rspan":1,"markup":[1,133]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8585560/}{Toward   developing a systematic approach to generate benchmark android malware   datasets and classification}","cspan":1,"rspan":1,"markup":[1,172]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9206660/}{On   the (un) reliability of privacy policies in android apps}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-93411-2_4}{Honey,   i shrunk your app security: The state of android app hardening}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.mdpi.com/2073-8994/12/7/1128}{Two   Anatomists Are Better than One—Dual-Level Android Malware Detection}","cspan":1,"rspan":1,"markup":[1,122]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9286110/}{An   Automated Assessment of Android Clipboards}","cspan":1,"rspan":1,"markup":[1,110]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://i.blackhat.com/us-18/Thu-August-9/us-18-Schranz-ARTist-A-Novel-Instrumentation-Framework-for-Reversing-and-Analyzing-Android-Apps-and-the-Middleware.pdf}{ARTist-A   novel ins trumentation framework for reversing and analyzing android apps and   the middleware}","cspan":1,"rspan":1,"markup":[1,274]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://publications.cispa.saarland/id/eprint/3340}{Bringing   Balance to the Force: Dynamic Analysis of the Android Application Framework}","cspan":1,"rspan":1,"markup":[1,145]},{"value":"2021","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-44038-1_120}{Android   Hook Detection Based on Machine Learning and Dynamic Analysis}","cspan":1,"rspan":1,"markup":[1,143]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://essay.utwente.nl/79200/}{Remote   runtime detection of tampering and of dynamic analysis attempts for Android   apps}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.diva-portal.org/smash/record.jsf?pid=diva2:1109568}{Evaluating   Dynamic AnalysisMethods for Android Applications}","cspan":1,"rspan":1,"markup":[1,132]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.usenix.org/conference/raid2019/presentation/nisi}{Exploring   Syscall-Based Semantics Reconstruction of Android Applications}","cspan":1,"rspan":1,"markup":[1,143]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-981-15-9609-4_7}{A   Hidden File Extraction Scheme Defeating Malware Using Android Dynamic   Loading}","cspan":1,"rspan":1,"markup":[1,153]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2857705.2857739}{Aspectdroid:   Android app analysis system}","cspan":1,"rspan":1,"markup":[1,101]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7502337/}{DynaLog:   An automated dynamic analysis framework for characterizing android   applications}","cspan":1,"rspan":1,"markup":[1,155]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s10586-016-0703-5}{Droidward:   an effective dynamic analysis method for vetting android applications}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7417621/}{Reevaluating   android permission gaps with static and dynamic analysis}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.ndss-symposium.org/wp-content/uploads/2017/09/intellidroid-targeted-input-generator-dynamic-analysis-android-malware.pdf}{IntelliDroid:   A Targeted Input Generator for the Dynamic Analysis of Android Malware.}","cspan":1,"rspan":1,"markup":[1,228]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3212480.3212504}{Towards   dynamically monitoring Android applications on non-rooted devices in the   wild}","cspan":1,"rspan":1,"markup":[1,148]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.mdpi.com/558048}{AndroShield:   automated android applications vulnerability detection, a hybrid static and   dynamic analysis approach}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7226692/}{Code   coverage measurement for Android dynamic analysis tools}","cspan":1,"rspan":1,"markup":[1,125]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6906344/}{DroidTrace:   A ptrace based Android dynamic analysis system with forward execution   capability}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7898406/}{Security   assessment of code obfuscation based on dynamic monitoring in android things}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2663761.2664223}{DroidDolphin:   a dynamic Android malware detection framework using big data and machine   learning}","cspan":1,"rspan":1,"markup":[1,158]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-981-15-1675-7_2}{The   state of Android security}","cspan":1,"rspan":1,"markup":[1,101]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=72nnDwAAQBAJ&oi=fnd&pg=PA73&dq=android+dynamic+analysis+api+monitoring&ots=42pKkKSqp8&sig=w0EpaqnSTh9vXWgcjOYUCnLmkxY}{Effectiveness   of state-of-the-art dynamic analysis techniques in identifying diverse   Android malware and future enhancements}","cspan":1,"rspan":1,"markup":[1,298]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2592791.2592796}{Rage   against the virtual machine: hindering dynamic analysis of android malware}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S1877050916001599}{Analysis   of malicious behavior of android apps}","cspan":1,"rspan":1,"markup":[1,124]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167404817301207}{DroidInjector:   A process injection-based dynamic tracking system for runtime behaviors of   Android applications}","cspan":1,"rspan":1,"markup":[1,190]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://ijns.jalaxy.com.tw/contents/ijns-v18-n1/ijns-2016-v18-n1-p182-192.pdf}{Malicious   behavior analysis for android applications}","cspan":1,"rspan":1,"markup":[1,139]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8374030/}{A   novel dynamic Android malware detection system with ensemble learning}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=rBMqCgAAQBAJ&oi=fnd&pg=PA93&dq=android+dynamic+analysis+api+monitoring&ots=g2qvPymWkq&sig=udNLczIfTd7rrN0JUfjt6v6Vl9I}{DroidMonitor:   a high-level programming model for dynamic API monitoring on Android}","cspan":1,"rspan":1,"markup":[1,254]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2480362.2480701}{Mobile-sandbox:   having a deeper look into android applications}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6906344/}{DroidTrace:   A ptrace based Android dynamic analysis system with forward execution   capability}","cspan":1,"rspan":1,"markup":[1,159]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://link.springer.com/article/10.1007/s10586-016-0703-5}{Droidward:   an effective dynamic analysis method for vetting android applications}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8706349/}{Real   time android ransomware detection by analyzed android applications}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.ndss-symposium.org/wp-content/uploads/2017/09/intellidroid-targeted-input-generator-dynamic-analysis-android-malware.pdf}{IntelliDroid:   A Targeted Input Generator for the Dynamic Analysis of Android Malware.}","cspan":1,"rspan":1,"markup":[1,228]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3212480.3212504}{Towards   dynamically monitoring Android applications on non-rooted devices in the   wild}","cspan":1,"rspan":1,"markup":[1,148]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2857705.2857739}{Aspectdroid:   Android app analysis system}","cspan":1,"rspan":1,"markup":[1,101]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8374030/}{A   novel dynamic Android malware detection system with ensemble learning}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8255546/}{Samadroid:   a novel 3-level hybrid malware detection model for android operating system}","cspan":1,"rspan":1,"markup":[1,151]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S074373151630140X}{A   hybrid approach of mobile malware detection in Android}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8074847/}{Malware   detection in android based on dynamic analysis}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.1073.3909&rep=rep1&type=pdf}{Android   based mobile application development and its security}","cspan":1,"rspan":1,"markup":[1,157]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S2214212619303837}{Visualizing   the outcome of dynamic analysis of Android malware with VizMal}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{http://ceur-ws.org/Vol-1575/paper_10.pdf}{ARTDroid:   A Virtual-Method Hooking Framework on Android ART Runtime.}","cspan":1,"rspan":1,"markup":[1,119]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2480362.2480701}{Mobile-sandbox:   having a deeper look into android applications}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://books.google.com/books?hl=en&lr=&id=72nnDwAAQBAJ&oi=fnd&pg=PA73&dq=android+dynamic+analysis+file+access+monitoring&ots=42pKkKSqr5&sig=nrqD9lZkPLoM6xuvqojzkmqQ1O0}{Effectiveness   of state-of-the-art dynamic analysis techniques in identifying diverse   Android malware and future enhancements}","cspan":1,"rspan":1,"markup":[1,306]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2619239.2631434}{Droid-sec:   deep learning in android malware detection}","cspan":1,"rspan":1,"markup":[1,114]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.mdpi.com/558048}{AndroShield:   automated android applications vulnerability detection, a hybrid static and   dynamic analysis approach}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2046614.2046619}{Crowdroid:   behavior-based malware detection system for android}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2011","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7417621/}{Reevaluating   android permission gaps with static and dynamic analysis}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2614628.2614633}{Android   taint flow analysis for app sets}","cspan":1,"rspan":1,"markup":[1,101]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6394931/}{Leakminer:   Detect information leakage on android with static taint analysis}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2666356.2594299}{Flowdroid:   Precise context, flow, field, object-sensitive and lifecycle-aware taint   analysis for android apps}","cspan":1,"rspan":1,"markup":[1,172]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://orbilu.uni.lu/bitstream/10993/25162/1/Highly%20Precise%20Taint%20Analysis%20for%20Android%20Application.pdf}{Highly   precise taint analysis for android applications}","cspan":1,"rspan":1,"markup":[1,180]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3236024.3236029}{Do   android taint analysis tools keep their promises?}","cspan":1,"rspan":1,"markup":[1,113]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2771783.2771803}{Scalable   and precise taint analysis for android}","cspan":1,"rspan":1,"markup":[1,108]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://arxiv.org/abs/1404.7431}{I   know what leaked in your pocket: uncovering privacy leaks on Android Apps   with Static Taint Analysis}","cspan":1,"rspan":1,"markup":[1,146]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8952502/}{A   qualitative analysis of Android taint-analysis results}","cspan":1,"rspan":1,"markup":[1,121]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/2635868.2635869}{Apposcopy:   Semantics-based detection of android malware through static analysis}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7582763/}{HybriDroid:   static analysis framework for Android hybrid applications}","cspan":1,"rspan":1,"markup":[1,134]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0950584917302987}{Static   analysis of android apps: A systematic literature review}","cspan":1,"rspan":1,"markup":[1,141]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8010886/}{TaintMan:   An ART-compatible dynamic taint analysis framework on unmodified and   non-rooted Android devices}","cspan":1,"rspan":1,"markup":[1,172]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6461017/}{TrustDroid:   Preventing the use of SmartPhones for information leaking in corporate   networks through the used of static analysis taint tracking}","cspan":1,"rspan":1,"markup":[1,209]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/9284080/}{Heaps'n   leaks: how heap snapshots improve Android taint analysis}","cspan":1,"rspan":1,"markup":[1,129]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7011272/}{Appcaulk:   Data leak prevention by injecting targeted taint tracking into android apps}","cspan":1,"rspan":1,"markup":[1,150]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8410576/}{BridgeTaint:   a bi-directional dynamic taint tracking method for JavaScript bridges in   android hybrid applications}","cspan":1,"rspan":1,"markup":[1,180]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/7223198/}{On   the effectiveness of dynamic taint analysis for protecting against private   information leaks on Android-based devices}","cspan":1,"rspan":1,"markup":[1,187]},{"value":"2013","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3196398.3196433}{Leveraging   historical versions of Android apps for efficient and precise taint analysis}","cspan":1,"rspan":1,"markup":[1,148]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6828062/}{Overview   of information flow tracking techniques based on taint analysis for android}","cspan":1,"rspan":1,"markup":[1,149]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3243218.3243222}{Poking   the bear: Lessons learned from probing three android malware datasets}","cspan":1,"rspan":1,"markup":[1,137]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-58469-0_23}{Binsign:   fingerprinting binary functions to support automated analysis of code   executables}","cspan":1,"rspan":1,"markup":[1,165]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity12/technical-sessions/presentation/yan}{Droidscope:   Seamlessly reconstructing the OS and dalvik semantic views for dynamic   android malware analysis}","cspan":1,"rspan":1,"markup":[1,206]},{"value":"2012","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S016740481630164X}{DroidNative:   Automating and optimizing detection of Android native code malware variants}","cspan":1,"rspan":1,"markup":[1,166]},{"value":"2017","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://arxiv.org/abs/1903.10560}{Don't   Pick the Cherry: An Evaluation Methodology for Android Malware Detection   Methods}","cspan":1,"rspan":1,"markup":[1,131]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3319535.3354240}{Automatic   fingerprinting of vulnerable ble iot devices with static uuids from mobile   apps}","cspan":1,"rspan":1,"markup":[1,152]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8514207/}{Unmasking   android obfuscation tools using spatial analysis}","cspan":1,"rspan":1,"markup":[1,123]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://dl.acm.org/doi/abs/10.1145/3176258.3176322}{Authorship   attribution of android apps}","cspan":1,"rspan":1,"markup":[1,99]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://core.ac.uk/download/pdf/286999186.pdf}{Obfuscation   fingerprinting in Android binaries}","cspan":1,"rspan":1,"markup":[1,102]},{"value":"2015","cspan":1,"rspan":1,"markup":[1,4]},{"value":"TRUE","cspan":1,"rspan":1,"markup":[1,4]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/6999911/}{Android   security: a survey of issues, malware penetration, and defenses}","cspan":1,"rspan":1,"markup":[1,136]},{"value":"2014","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.usenix.org/conference/usenixsecurity19/presentation/pham}{Hidemyapp:   Hiding the presence of sensitive apps on android}","cspan":1,"rspan":1,"markup":[1,138]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167404817302377}{Toward   a more dependable hybrid analysis of android malware using aspect-oriented   programming}","cspan":1,"rspan":1,"markup":[1,173]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-030-34238-8_3}{Compiler   Provenance Attribution}","cspan":1,"rspan":1,"markup":[1,103]},{"value":"2020","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://ieeexplore.ieee.org/abstract/document/8684307/}{EveDroid:   Event-aware Android malware detection against model degrading for IoT   devices}","cspan":1,"rspan":1,"markup":[1,154]},{"value":"2019","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://link.springer.com/chapter/10.1007/978-3-319-59608-2_3}{Exploiting   android system services through bypassing service helpers}","cspan":1,"rspan":1,"markup":[1,140]},{"value":"2016","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"\\href{https://www.sciencedirect.com/science/article/pii/S0167739X17329965}{Big   Data fingerprinting information analytics for sustainability}","cspan":1,"rspan":1,"markup":[1,142]},{"value":"2018","cspan":1,"rspan":1,"markup":[1,4]},{"value":"FALSE","cspan":1,"rspan":1,"markup":[1,5]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":""}}]},"options":{"table_caption":"","table_label":"tab:my-table"}}

==> assets/Tables/MalwareFirmwares <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Packagename","cspan":1,"rspan":1,"markup":[2,11]},{"value":"MD5","cspan":1,"rspan":1,"markup":[2,3]},{"value":"Firmware\nBrand\n(ro.build.brand)","cspan":1,"rspan":1,"markup":[1,31]},{"value":"Firmware \nbuild key\n(ro.build.tags)","cspan":1,"rspan":1,"markup":[1,35]}],[{"value":"com.transsion.statisticalsales","cspan":1,"rspan":1,"markup":[1,30]},{"value":"a24f48fcd9f390800640a9d34b369c6c ","cspan":1,"rspan":1,"markup":[1,33]},{"value":"Tecno","cspan":1,"rspan":1,"markup":[1,5]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.customermobile.preload.vzw","cspan":1,"rspan":1,"markup":[1,30]},{"value":"5a8913dc5df6a14b2673286b04b12539   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Google","cspan":1,"rspan":1,"markup":[1,6]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.m2fpremium.furiousthief","cspan":1,"rspan":1,"markup":[1,27]},{"value":"0bd71ad1afe8df86e289f0c89609898f   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Micromax","cspan":1,"rspan":1,"markup":[1,8]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.gameneeti.game.MissionSpaceGN1Pro   ","cspan":1,"rspan":1,"markup":[1,40]},{"value":"419d00d77fcc50e03e2b95ff8d56def0   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Micromax","cspan":1,"rspan":1,"markup":[1,8]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.smart.weather   ","cspan":1,"rspan":1,"markup":[1,20]},{"value":"5f6b1cdcb4ea5ca0e973a081a4b0c6c4   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Imkj","cspan":1,"rspan":1,"markup":[1,4]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.cooee.phenix   ","cspan":1,"rspan":1,"markup":[1,19]},{"value":"bd44a85905c7ee2264a08b26ef1c7527   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Imkj","cspan":1,"rspan":1,"markup":[1,4]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.zte.zdm","cspan":1,"rspan":1,"markup":[1,11]},{"value":"be81670b117cad27d04de61cb3aed17d   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"ZTE","cspan":1,"rspan":1,"markup":[1,3]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.google.speed.anisotropic.multistage   ","cspan":1,"rspan":1,"markup":[1,42]},{"value":"3cb9b635fd5b2b3d134bbe55194b4fa0   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Allview","cspan":1,"rspan":1,"markup":[1,7]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.aptoide.partners.id3storen   ","cspan":1,"rspan":1,"markup":[1,33]},{"value":"2fd47f2a914da16fa7f2b933a15e7808   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Nokia","cspan":1,"rspan":1,"markup":[1,5]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.excelliance.dualaid.vend   ","cspan":1,"rspan":1,"markup":[1,31]},{"value":"af7a90c7403555b04f53193ae25f1c0d   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Infinix","cspan":1,"rspan":1,"markup":[1,7]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.vivo.globalsearch   ","cspan":1,"rspan":1,"markup":[1,24]},{"value":"fab5f84300876e0920dbf96b0c86aa32   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Vivo","cspan":1,"rspan":1,"markup":[1,4]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.bbk.theme   ","cspan":1,"rspan":1,"markup":[1,16]},{"value":"3010ce4b192d57fc26e2c32a3374d423   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Vivo","cspan":1,"rspan":1,"markup":[1,4]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.mobile.iroaming   ","cspan":1,"rspan":1,"markup":[1,22]},{"value":"5d97ad886275c28534b9ea253be4354e   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Vivo","cspan":1,"rspan":1,"markup":[1,4]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.synchronoss.dcs.att.r2g   ","cspan":1,"rspan":1,"markup":[1,30]},{"value":"a10bf6bc3c0c7ca4e37395666a22ec29   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Samsung","cspan":1,"rspan":1,"markup":[1,7]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.android.sales   ","cspan":1,"rspan":1,"markup":[1,20]},{"value":"034ff8ce04cb7ab38fe455a4fe1682c3   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Lava","cspan":1,"rspan":1,"markup":[1,4]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.gameneeti.game.aliensmarsfightpro   ","cspan":1,"rspan":1,"markup":[1,40]},{"value":"a652a9e1fb949341ae247e1c985a85c2   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Symphony","cspan":1,"rspan":1,"markup":[1,8]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.cmcc.cmvideo   ","cspan":1,"rspan":1,"markup":[1,19]},{"value":"2dee8d84291398f354f92629b759fca7   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Samsung","cspan":1,"rspan":1,"markup":[1,7]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.aspire.mm   ","cspan":1,"rspan":1,"markup":[1,16]},{"value":"ed73284f6ec22486453fa92987e61b5a   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Samsung","cspan":1,"rspan":1,"markup":[1,7]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"cmccwm.mobilemusic   ","cspan":1,"rspan":1,"markup":[1,21]},{"value":"a7a4a4720537395b45d5e14d2c777a1c   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Samsung","cspan":1,"rspan":1,"markup":[1,7]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.digi10soft.game.letsplay2020pro   ","cspan":1,"rspan":1,"markup":[1,38]},{"value":"2d1c3e78fed97ef51adfedc54b797017   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Micromax","cspan":1,"rspan":1,"markup":[1,8]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.samsung.android.mobileservice   ","cspan":1,"rspan":1,"markup":[1,36]},{"value":"274a15289edca85044eadd443c362e6c   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Samsung","cspan":1,"rspan":1,"markup":[1,7]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.sina.weibo   ","cspan":1,"rspan":1,"markup":[1,17]},{"value":"8a9d1b85e613306e7830ddad92afd69a   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Samsung","cspan":1,"rspan":1,"markup":[1,7]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.dti.att   ","cspan":1,"rspan":1,"markup":[1,14]},{"value":"e04e0fae2f9ef13599ddd4c978b95cd0   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Samsung","cspan":1,"rspan":1,"markup":[1,7]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.vzw.ecid   ","cspan":1,"rspan":1,"markup":[1,15]},{"value":"3f0e107d7b8dbc583fea1352f5e7b7d7   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Samsung","cspan":1,"rspan":1,"markup":[1,7]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.emoji.keyboard.touchpal.vivo   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"a812de7cdd6692380c81a0348ba312a4   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Vivo","cspan":1,"rspan":1,"markup":[1,4]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":""}},null]},"options":{"table_caption":"Malware samples with corresponding brand and key.","table_label":"tab:MalwareFirmwareBrands"}}

==> assets/Tables/TLSH_eval_10000 <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Band \nWidth \nThreshold","cspan":1,"rspan":1,"markup":[2,22]},{"value":"Table \ncreation \ntime (s)","cspan":1,"rspan":1,"markup":[2,25]},{"value":"Cluster \ncreation \ntime (s)","cspan":1,"rspan":1,"markup":[2,27]},{"value":"Total \ntime (s)","cspan":1,"rspan":1,"markup":[2,15]},{"value":"Group \nsize\naverage","cspan":1,"rspan":1,"markup":[2,19]},{"value":"Number \nof\nclusters","cspan":1,"rspan":1,"markup":[2,19]},{"value":"Group \ndifference","cspan":1,"rspan":1,"markup":[2,17]},{"value":"Number \nof \ncomparisons\n(decrease rate)","cspan":1,"rspan":1,"markup":[1,39]},{"value":"Comparisons \ndifference","cspan":1,"rspan":1,"markup":[2,23]},{"value":"Missed \nrate","cspan":1,"rspan":1,"markup":[2,12]},{"value":"Hit \nrate","cspan":1,"rspan":1,"markup":[2,9]}],[{"value":"1","cspan":1,"rspan":1,"markup":[2,1]},{"value":"3'475","cspan":1,"rspan":1,"markup":[1,5]},{"value":"58'162","cspan":1,"rspan":1,"markup":[1,6]},{"value":"61'637","cspan":1,"rspan":1,"markup":[1,6]},{"value":"7.3913","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'076","cspan":1,"rspan":1,"markup":[1,5]},{"value":"0","cspan":1,"rspan":1,"markup":[1,1]},{"value":"99'436'120 (0.56%)","cspan":1,"rspan":1,"markup":[1,18]},{"value":"563'880","cspan":1,"rspan":1,"markup":[1,7]},{"value":"0","cspan":1,"rspan":1,"markup":[1,1]},{"value":"7'953","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"5","cspan":1,"rspan":1,"markup":[2,1]},{"value":"3'304","cspan":1,"rspan":1,"markup":[1,5]},{"value":"46'295","cspan":1,"rspan":1,"markup":[1,6]},{"value":"49'599","cspan":1,"rspan":1,"markup":[1,6]},{"value":"7.3913","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'076","cspan":1,"rspan":1,"markup":[1,5]},{"value":"0","cspan":1,"rspan":1,"markup":[1,1]},{"value":"61'719'110 (38.28%)","cspan":1,"rspan":1,"markup":[1,19]},{"value":"38'280'890","cspan":1,"rspan":1,"markup":[1,10]},{"value":"0","cspan":1,"rspan":1,"markup":[1,1]},{"value":"7'953","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"10","cspan":1,"rspan":1,"markup":[2,2]},{"value":"3'298","cspan":1,"rspan":1,"markup":[1,5]},{"value":"12'219","cspan":1,"rspan":1,"markup":[1,6]},{"value":"15'517","cspan":1,"rspan":1,"markup":[1,6]},{"value":"7.3903","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'076","cspan":1,"rspan":1,"markup":[1,5]},{"value":"0","cspan":1,"rspan":1,"markup":[1,1]},{"value":"8'598'052 (91.4%)","cspan":1,"rspan":1,"markup":[1,17]},{"value":"91'401'948","cspan":1,"rspan":1,"markup":[1,10]},{"value":"1 (0.01%)","cspan":1,"rspan":1,"markup":[1,9]},{"value":"7'952","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"11","cspan":1,"rspan":1,"markup":[2,2]},{"value":"3'278","cspan":1,"rspan":1,"markup":[1,5]},{"value":"9'290","cspan":1,"rspan":1,"markup":[1,5]},{"value":"12'568","cspan":1,"rspan":1,"markup":[1,6]},{"value":"7.3935","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'075","cspan":1,"rspan":1,"markup":[1,5]},{"value":"1","cspan":1,"rspan":1,"markup":[1,1]},{"value":"5'606'898 (94.39%)","cspan":1,"rspan":1,"markup":[1,18]},{"value":"94'393'102","cspan":1,"rspan":1,"markup":[1,10]},{"value":"5 (0.06%)","cspan":1,"rspan":1,"markup":[1,9]},{"value":"7'948","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"12","cspan":1,"rspan":1,"markup":[2,2]},{"value":"3'300","cspan":1,"rspan":1,"markup":[1,5]},{"value":"7'401","cspan":1,"rspan":1,"markup":[1,5]},{"value":"10'701","cspan":1,"rspan":1,"markup":[1,6]},{"value":"7.3907","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'075","cspan":1,"rspan":1,"markup":[1,5]},{"value":"1","cspan":1,"rspan":1,"markup":[1,1]},{"value":"3'848'412 (96.15%)","cspan":1,"rspan":1,"markup":[1,18]},{"value":"96'151'588","cspan":1,"rspan":1,"markup":[1,10]},{"value":"8 (0.1%)","cspan":1,"rspan":1,"markup":[1,8]},{"value":"7'945","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"13","cspan":1,"rspan":1,"markup":[2,2]},{"value":"3'275","cspan":1,"rspan":1,"markup":[1,5]},{"value":"6'207","cspan":1,"rspan":1,"markup":[1,5]},{"value":"9'483","cspan":1,"rspan":1,"markup":[1,5]},{"value":"7.3736","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'076","cspan":1,"rspan":1,"markup":[1,5]},{"value":"0","cspan":1,"rspan":1,"markup":[1,1]},{"value":"2'829'730 (97.17%)","cspan":1,"rspan":1,"markup":[1,18]},{"value":"97'170'270","cspan":1,"rspan":1,"markup":[1,10]},{"value":"19 (0.24%)","cspan":1,"rspan":1,"markup":[1,10]},{"value":"7'934","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"15","cspan":1,"rspan":1,"markup":[2,2]},{"value":"3'283","cspan":1,"rspan":1,"markup":[1,5]},{"value":"4'949","cspan":1,"rspan":1,"markup":[1,5]},{"value":"8'232","cspan":1,"rspan":1,"markup":[1,5]},{"value":"7.2631","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'087","cspan":1,"rspan":1,"markup":[1,5]},{"value":"11","cspan":1,"rspan":1,"markup":[1,2]},{"value":"1'863'104 (98.14%)","cspan":1,"rspan":1,"markup":[1,18]},{"value":"98'136'896","cspan":1,"rspan":1,"markup":[1,10]},{"value":"58 (0.73%)","cspan":1,"rspan":1,"markup":[1,10]},{"value":"7'895","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"18","cspan":1,"rspan":1,"markup":[2,2]},{"value":"3'266","cspan":1,"rspan":1,"markup":[1,5]},{"value":"3'893","cspan":1,"rspan":1,"markup":[1,5]},{"value":"7'159","cspan":1,"rspan":1,"markup":[1,5]},{"value":"6.8627","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'129","cspan":1,"rspan":1,"markup":[1,5]},{"value":"53","cspan":1,"rspan":1,"markup":[1,2]},{"value":"1'220'616 (98.78%)","cspan":1,"rspan":1,"markup":[1,18]},{"value":"98'779'384","cspan":1,"rspan":1,"markup":[1,10]},{"value":"205 (2.58%)","cspan":1,"rspan":1,"markup":[1,11]},{"value":"7'748","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"20","cspan":1,"rspan":1,"markup":[2,2]},{"value":"3'291","cspan":1,"rspan":1,"markup":[1,5]},{"value":"3'281","cspan":1,"rspan":1,"markup":[1,5]},{"value":"6'572","cspan":1,"rspan":1,"markup":[1,5]},{"value":"6.4855","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'170","cspan":1,"rspan":1,"markup":[1,5]},{"value":"94","cspan":1,"rspan":1,"markup":[1,2]},{"value":"924'320 (99.08%)","cspan":1,"rspan":1,"markup":[1,16]},{"value":"99'075'680","cspan":1,"rspan":1,"markup":[1,10]},{"value":"365 (4.59%)","cspan":1,"rspan":1,"markup":[1,11]},{"value":"7'588","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"30","cspan":1,"rspan":1,"markup":[2,2]},{"value":"3'255","cspan":1,"rspan":1,"markup":[1,5]},{"value":"1'194","cspan":1,"rspan":1,"markup":[1,5]},{"value":"4'448","cspan":1,"rspan":1,"markup":[1,5]},{"value":"4.5269","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'395","cspan":1,"rspan":1,"markup":[1,5]},{"value":"319","cspan":1,"rspan":1,"markup":[1,3]},{"value":"142'016 (99.86%)","cspan":1,"rspan":1,"markup":[1,16]},{"value":"99'857'984","cspan":1,"rspan":1,"markup":[1,10]},{"value":"1'638 (20.6%)","cspan":1,"rspan":1,"markup":[1,13]},{"value":"6'315","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"40","cspan":1,"rspan":1,"markup":[2,2]},{"value":"3'295","cspan":1,"rspan":1,"markup":[1,5]},{"value":"933","cspan":1,"rspan":1,"markup":[1,3]},{"value":"4'228","cspan":1,"rspan":1,"markup":[1,5]},{"value":"3.8449","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'354","cspan":1,"rspan":1,"markup":[1,5]},{"value":"278","cspan":1,"rspan":1,"markup":[1,3]},{"value":"83'332 (99.92%)","cspan":1,"rspan":1,"markup":[1,15]},{"value":"99'916'668","cspan":1,"rspan":1,"markup":[1,10]},{"value":"2'747 (34.54%)","cspan":1,"rspan":1,"markup":[1,14]},{"value":"5'206","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"50","cspan":1,"rspan":1,"markup":[2,2]},{"value":"3'302","cspan":1,"rspan":1,"markup":[1,5]},{"value":"799","cspan":1,"rspan":1,"markup":[1,3]},{"value":"4'102","cspan":1,"rspan":1,"markup":[1,5]},{"value":"3.7365","cspan":1,"rspan":1,"markup":[1,6]},{"value":"1'237","cspan":1,"rspan":1,"markup":[1,5]},{"value":"161","cspan":1,"rspan":1,"markup":[1,3]},{"value":"64'442 (99.94%)","cspan":1,"rspan":1,"markup":[1,15]},{"value":"99'935'558","cspan":1,"rspan":1,"markup":[1,10]},{"value":"3'331 (41.88%)","cspan":1,"rspan":1,"markup":[1,14]},{"value":"4'622","cspan":1,"rspan":1,"markup":[1,5]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":""}}]},"options":{"table_caption":"Performance measurement for 10'000 TLSH hashes with variable band width thresholds.","table_label":"tab:TLSH_eval_10000"}}

==> assets/Tables/TLSH_eval_5000 <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"font-weight":"normal"},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Band \nWidth \nThreshold","cspan":1,"rspan":1,"markup":[2,22]},{"value":"Table \ncreation \ntime (s)","cspan":1,"rspan":1,"markup":[2,25]},{"value":"Cluster \ncreation \ntime (s)","cspan":1,"rspan":1,"markup":[2,27]},{"value":"Total \ntime (s)","cspan":1,"rspan":1,"markup":[2,15]},{"value":"Group \nsize\naverage","cspan":1,"rspan":1,"markup":[2,19]},{"value":"Number \nof\nclusters","cspan":1,"rspan":1,"markup":[2,19]},{"value":"Group \ndifference","cspan":1,"rspan":1,"markup":[2,17]},{"value":"Number \nof \ncomparisons \n(decrease rate)","cspan":1,"rspan":1,"markup":[1,40]},{"value":"Comparisons \ndifference","cspan":1,"rspan":1,"markup":[2,23]},{"value":"Missed \nrate","cspan":1,"rspan":1,"markup":[2,12]},{"value":"Hit \nrate","cspan":1,"rspan":1,"markup":[2,9]}],[{"value":"5","cspan":1,"rspan":1,"markup":[2,1]},{"value":"502","cspan":1,"rspan":1,"markup":[1,3]},{"value":"5'724","cspan":1,"rspan":1,"markup":[1,5]},{"value":"6'226","cspan":1,"rspan":1,"markup":[1,5]},{"value":"9.4052","cspan":1,"rspan":1,"markup":[1,6]},{"value":"427","cspan":1,"rspan":1,"markup":[1,3]},{"value":"0","cspan":1,"rspan":1,"markup":[1,1]},{"value":"15'967'554 (36.13%}","cspan":1,"rspan":1,"markup":[1,19]},{"value":"9'032'446","cspan":1,"rspan":1,"markup":[1,9]},{"value":"0 (0%)","cspan":1,"rspan":1,"markup":[1,6]},{"value":"4'016","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"10","cspan":1,"rspan":1,"markup":[2,2]},{"value":"481","cspan":1,"rspan":1,"markup":[1,3]},{"value":"1'951","cspan":1,"rspan":1,"markup":[1,5]},{"value":"2'432","cspan":1,"rspan":1,"markup":[1,5]},{"value":"9.3832","cspan":1,"rspan":1,"markup":[1,6]},{"value":"428","cspan":1,"rspan":1,"markup":[1,3]},{"value":"1","cspan":1,"rspan":1,"markup":[1,1]},{"value":"3'004'622 (87.98%)","cspan":1,"rspan":1,"markup":[1,18]},{"value":"21'995'378","cspan":1,"rspan":1,"markup":[1,10]},{"value":"0 (0%)","cspan":1,"rspan":1,"markup":[1,6]},{"value":"4'016","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"13","cspan":1,"rspan":1,"markup":[2,2]},{"value":"500","cspan":1,"rspan":1,"markup":[1,3]},{"value":"1'114","cspan":1,"rspan":1,"markup":[1,5]},{"value":"1'614","cspan":1,"rspan":1,"markup":[1,5]},{"value":"9.2656","cspan":1,"rspan":1,"markup":[1,6]},{"value":"433","cspan":1,"rspan":1,"markup":[1,3]},{"value":"6","cspan":1,"rspan":1,"markup":[1,1]},{"value":"1'260'828 (94.96%)","cspan":1,"rspan":1,"markup":[1,18]},{"value":"23'739'172","cspan":1,"rspan":1,"markup":[1,10]},{"value":"4 (0.1%)","cspan":1,"rspan":1,"markup":[1,8]},{"value":"4'012","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"15","cspan":1,"rspan":1,"markup":[2,2]},{"value":"602","cspan":1,"rspan":1,"markup":[1,3]},{"value":"952","cspan":1,"rspan":1,"markup":[1,3]},{"value":"1'555","cspan":1,"rspan":1,"markup":[1,5]},{"value":"9.1050","cspan":1,"rspan":1,"markup":[1,6]},{"value":"438","cspan":1,"rspan":1,"markup":[1,3]},{"value":"11","cspan":1,"rspan":1,"markup":[1,2]},{"value":"835'422 (96.66%)","cspan":1,"rspan":1,"markup":[1,16]},{"value":"24'164'578","cspan":1,"rspan":1,"markup":[1,10]},{"value":"28 (0.67%)","cspan":1,"rspan":1,"markup":[1,10]},{"value":"3'988","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"18","cspan":1,"rspan":1,"markup":[2,2]},{"value":"514","cspan":1,"rspan":1,"markup":[1,3]},{"value":"870","cspan":1,"rspan":1,"markup":[1,3]},{"value":"1'384","cspan":1,"rspan":1,"markup":[1,5]},{"value":"8.3879","cspan":1,"rspan":1,"markup":[1,6]},{"value":"464","cspan":1,"rspan":1,"markup":[1,3]},{"value":"37","cspan":1,"rspan":1,"markup":[1,2]},{"value":"522'050 (97.91%)","cspan":1,"rspan":1,"markup":[1,16]},{"value":"24'477'950","cspan":1,"rspan":1,"markup":[1,10]},{"value":"124 (3.1%)","cspan":1,"rspan":1,"markup":[1,10]},{"value":"3'892","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"20","cspan":1,"rspan":1,"markup":[2,2]},{"value":"824","cspan":1,"rspan":1,"markup":[1,3]},{"value":"812","cspan":1,"rspan":1,"markup":[1,3]},{"value":"1'636","cspan":1,"rspan":1,"markup":[1,5]},{"value":"7.6343","cspan":1,"rspan":1,"markup":[1,6]},{"value":"495","cspan":1,"rspan":1,"markup":[1,3]},{"value":"68","cspan":1,"rspan":1,"markup":[1,2]},{"value":"396'178 (98.42%)","cspan":1,"rspan":1,"markup":[1,16]},{"value":"24'603'822","cspan":1,"rspan":1,"markup":[1,10]},{"value":"237 (5.9%)","cspan":1,"rspan":1,"markup":[1,10]},{"value":"3'779","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"30","cspan":1,"rspan":1,"markup":[2,2]},{"value":"722","cspan":1,"rspan":1,"markup":[1,3]},{"value":"351","cspan":1,"rspan":1,"markup":[1,3]},{"value":"1'073","cspan":1,"rspan":1,"markup":[1,5]},{"value":"4.5402","cspan":1,"rspan":1,"markup":[1,6]},{"value":"659","cspan":1,"rspan":1,"markup":[1,3]},{"value":"232","cspan":1,"rspan":1,"markup":[1,3]},{"value":"79'996 (99.68%)","cspan":1,"rspan":1,"markup":[1,15]},{"value":"24'920'004","cspan":1,"rspan":1,"markup":[1,10]},{"value":"1'024 (25,5%)","cspan":1,"rspan":1,"markup":[1,13]},{"value":"2'992","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"40","cspan":1,"rspan":1,"markup":[2,2]},{"value":"671","cspan":1,"rspan":1,"markup":[1,3]},{"value":"349","cspan":1,"rspan":1,"markup":[1,3]},{"value":"1'020","cspan":1,"rspan":1,"markup":[1,5]},{"value":"3.1567","cspan":1,"rspan":1,"markup":[1,6]},{"value":"804","cspan":1,"rspan":1,"markup":[1,3]},{"value":"377","cspan":1,"rspan":1,"markup":[1,3]},{"value":"55'940 (99.78%)","cspan":1,"rspan":1,"markup":[1,15]},{"value":"24'944'060","cspan":1,"rspan":1,"markup":[1,10]},{"value":"1'478 (36,8%)","cspan":1,"rspan":1,"markup":[1,13]},{"value":"2'538","cspan":1,"rspan":1,"markup":[1,5]}],[{"value":"50","cspan":1,"rspan":1,"markup":[2,2]},{"value":"692","cspan":1,"rspan":1,"markup":[1,3]},{"value":"193","cspan":1,"rspan":1,"markup":[1,3]},{"value":"886","cspan":1,"rspan":1,"markup":[1,3]},{"value":"2.9413","cspan":1,"rspan":1,"markup":[1,6]},{"value":"733","cspan":1,"rspan":1,"markup":[1,3]},{"value":"306","cspan":1,"rspan":1,"markup":[1,3]},{"value":"53'126 (99.79%)","cspan":1,"rspan":1,"markup":[1,15]},{"value":"24'946'874","cspan":1,"rspan":1,"markup":[1,10]},{"value":"1'860 (46,3%)","cspan":1,"rspan":1,"markup":[1,13]},{"value":"2'156","cspan":1,"rspan":1,"markup":[1,5]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":""}},null]},"options":{"table_caption":"Performance measurement for 5000 TLSH hashes with variable band width thresholds.","table_label":"tab:TLSH_eval_5000"}}

==> assets/Tables/TLSH_missed_rates <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#EFEFEF","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Band \nWidth \nThreshold","cspan":1,"rspan":1,"markup":[3,22]},{"value":"Missed rate -\n10'000\nfiles - 1#","cspan":1,"rspan":1,"markup":[3,31]},{"value":"Missed rate -\n10'000\nfiles - 2#","cspan":1,"rspan":1,"markup":[3,31]},{"value":"Missed rate - \n10'000\napks - 3#","cspan":1,"rspan":1,"markup":[3,31]},{"value":"Missed rate -\n11'000\nfiles - 4#","cspan":1,"rspan":1,"markup":[3,31]},{"value":"Missed rate -\n12'000\nfiles - 5#","cspan":1,"rspan":1,"markup":[3,31]},{"value":"Missed rate -\n13'000\nfiles - 6#","cspan":1,"rspan":1,"markup":[3,31]},{"value":"Missed rate -\n14'000\nfiles - 7#","cspan":1,"rspan":1,"markup":[3,31]}],[{"value":"12","cspan":1,"rspan":1,"markup":[3,2]},{"value":"8 (0.1%)","cspan":1,"rspan":1,"markup":[3,8]},{"value":"9 (0.11%)","cspan":1,"rspan":1,"markup":[3,9]},{"value":"9 (0.11%)","cspan":1,"rspan":1,"markup":[3,9]},{"value":"9 (0.09%)","cspan":1,"rspan":1,"markup":[3,9]},{"value":"10 (0.1%)","cspan":1,"rspan":1,"markup":[3,9]},{"value":"9 (0.08%)","cspan":1,"rspan":1,"markup":[3,9]},{"value":"11 (0.09%)","cspan":1,"rspan":1,"markup":[3,10]}],[{"value":"13","cspan":1,"rspan":1,"markup":[3,2]},{"value":"19 (0.24%)","cspan":1,"rspan":1,"markup":[3,10]},{"value":"22 (0.28%)","cspan":1,"rspan":1,"markup":[3,10]},{"value":"21 (0.26%)","cspan":1,"rspan":1,"markup":[3,10]},{"value":"21 (0.22%)","cspan":1,"rspan":1,"markup":[3,10]},{"value":"18 (0.18%)","cspan":1,"rspan":1,"markup":[3,10]},{"value":"21 (0.19%)","cspan":1,"rspan":1,"markup":[3,10]},{"value":"28 (0.24%)","cspan":1,"rspan":1,"markup":[3,10]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},null,null,{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},null]},"options":{"table_caption":"Measurements for the missed rate with increasing number of files.","table_label":"tab:MissedRate_14000"}}

==> assets/Tables/Virustotal_Malware_Firmware <==
{"rows_views":[[{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{"bold":true},"text_color":"","bg_color":"#efefef","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}],[{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"left","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}},{"style":{"borders":"ltrb","font_style":{},"text_color":"","bg_color":"","halign":"center","valign":"top","padding":{"top":10,"right":5,"bottom":10,"left":5},"border_color":""}}]],"model":{"rows":[[{"value":"Packagename","cspan":1,"rspan":1,"markup":[2,11]},{"value":"MD5","cspan":1,"rspan":1,"markup":[2,3]},{"value":"Firmware\nBrand","cspan":1,"rspan":1,"markup":[1,14]},{"value":"Firmware\nro.build.tag","cspan":1,"rspan":1,"markup":[2,21]}],[{"value":"com.transsion.statisticalsales","cspan":1,"rspan":1,"markup":[1,30]},{"value":"a24f48fcd9f390800640a9d34b369c6c ","cspan":1,"rspan":1,"markup":[1,33]},{"value":"Tecno","cspan":1,"rspan":1,"markup":[1,5]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":" com.customermobile.preload.vzw","cspan":1,"rspan":1,"markup":[1,31]},{"value":"5a8913dc5df6a14b2673286b04b12539   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Google","cspan":1,"rspan":1,"markup":[1,6]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":" com.m2fpremium.furiousthief   ","cspan":1,"rspan":1,"markup":[1,31]},{"value":"0bd71ad1afe8df86e289f0c89609898f   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Micromax","cspan":1,"rspan":1,"markup":[1,8]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.gameneeti.game.MissionSpaceGN1Pro   ","cspan":1,"rspan":1,"markup":[1,40]},{"value":"419d00d77fcc50e03e2b95ff8d56def0   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"Micromax","cspan":1,"rspan":1,"markup":[1,8]},{"value":"release-keys","cspan":1,"rspan":1,"markup":[1,12]}],[{"value":"com.smart.weather   ","cspan":1,"rspan":1,"markup":[1,20]},{"value":"5f6b1cdcb4ea5ca0e973a081a4b0c6c4   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.cooee.phenix   ","cspan":1,"rspan":1,"markup":[1,19]},{"value":"bd44a85905c7ee2264a08b26ef1c7527   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.zte.zdm","cspan":1,"rspan":1,"markup":[1,11]},{"value":"be81670b117cad27d04de61cb3aed17d   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.google.speed.anisotropic.multistage   ","cspan":1,"rspan":1,"markup":[1,42]},{"value":"3cb9b635fd5b2b3d134bbe55194b4fa0   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.aptoide.partners.id3storen   ","cspan":1,"rspan":1,"markup":[1,33]},{"value":"2fd47f2a914da16fa7f2b933a15e7808   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.excelliance.dualaid.vend   ","cspan":1,"rspan":1,"markup":[1,31]},{"value":"af7a90c7403555b04f53193ae25f1c0d   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.vivo.globalsearch   ","cspan":1,"rspan":1,"markup":[1,24]},{"value":"fab5f84300876e0920dbf96b0c86aa32   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.bbk.theme   ","cspan":1,"rspan":1,"markup":[1,16]},{"value":"3010ce4b192d57fc26e2c32a3374d423   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.mobile.iroaming   ","cspan":1,"rspan":1,"markup":[1,22]},{"value":"5d97ad886275c28534b9ea253be4354e   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.synchronoss.dcs.att.r2g   ","cspan":1,"rspan":1,"markup":[1,30]},{"value":"a10bf6bc3c0c7ca4e37395666a22ec29   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.android.sales   ","cspan":1,"rspan":1,"markup":[1,20]},{"value":"034ff8ce04cb7ab38fe455a4fe1682c3   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.gameneeti.game.aliensmarsfightpro   ","cspan":1,"rspan":1,"markup":[1,40]},{"value":"a652a9e1fb949341ae247e1c985a85c2   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.cmcc.cmvideo   ","cspan":1,"rspan":1,"markup":[1,19]},{"value":"2dee8d84291398f354f92629b759fca7   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.aspire.mm   ","cspan":1,"rspan":1,"markup":[1,16]},{"value":"ed73284f6ec22486453fa92987e61b5a   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"cmccwm.mobilemusic   ","cspan":1,"rspan":1,"markup":[1,21]},{"value":"a7a4a4720537395b45d5e14d2c777a1c   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.digi10soft.game.letsplay2020pro   ","cspan":1,"rspan":1,"markup":[1,38]},{"value":"2d1c3e78fed97ef51adfedc54b797017   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.samsung.android.mobileservice   ","cspan":1,"rspan":1,"markup":[1,36]},{"value":"274a15289edca85044eadd443c362e6c   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.sina.weibo   ","cspan":1,"rspan":1,"markup":[1,17]},{"value":"8a9d1b85e613306e7830ddad92afd69a   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.dti.att   ","cspan":1,"rspan":1,"markup":[1,14]},{"value":"e04e0fae2f9ef13599ddd4c978b95cd0   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.vzw.ecid   ","cspan":1,"rspan":1,"markup":[1,15]},{"value":"3f0e107d7b8dbc583fea1352f5e7b7d7   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}],[{"value":"com.emoji.keyboard.touchpal.vivo   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"a812de7cdd6692380c81a0348ba312a4   ","cspan":1,"rspan":1,"markup":[1,35]},{"value":"","cspan":1,"rspan":1,"markup":[]},{"value":"","cspan":1,"rspan":1,"markup":[]}]]},"theme":null,"fixed_layout":false,"markup":{"instances":[{},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":"","backgroundColor":""}},{"style":{"fontWeight":"","fontStyle":"","textDecoration":"","color":""}},null]},"options":{"table_caption":"","table_label":"tab:my-table"}}

==> content/06_bloatware.tex <==









==> content/06_dataset.tex <==































==> content/11_future_work.tex <==




==> content/xx_results.tex <==
\chapter{Results and Discussion}\label{Results}

\section{Project Goals}

\section{Discussion}

\section{Future Work and Ideas}

\subsection{Contact Cards}

\section{Closing Remarks}

